Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation

Denoising Diffusion Probabilistic Model (DDPM) is able to make flexible conditional image generation from prior noise to real data, by introducing an independent noise-aware classifier to provide conditional gradient guidance at each time step of denoising process. However, due to the ability of classifier to easily discriminate an incompletely generated image only with high-level structure, the gradient, which is a kind of class information guidance, tends to vanish early, leading to the collapse from conditional generation process into the unconditional process. To address this problem, we propose two simple but effective approaches from two perspectives. For sampling procedure, we introduce the entropy of predicted distribution as the measure of guidance vanishing level and propose an entropy-aware scaling method to adaptively recover the conditional semantic guidance. For training stage, we propose the entropy-aware optimization objectives to alleviate the overconfident prediction for noisy data.On ImageNet1000 256x256, with our proposed sampling scheme and trained classifier, the pretrained conditional and unconditional DDPM model can achieve 10.89% (4.59 to 4.09) and 43.5% (12 to 6.78) FID improvement respectively. The code is available at https://github.com/ZGCTroy/ED-DPM.

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/0-asbtrast.tex <==
\begin{abstract}
    Denoising Diffusion Probabilistic Model (DDPM) is able to make flexible conditional image generation from prior noise to real data, by introducing an independent noise-aware classifier to provide conditional gradient guidance at each time step of denoising process.
    However, due to the ability of classifier to easily discriminate an incompletely generated image only with high-level structure, the gradient, which is a kind of class information guidance, tends to vanish early, leading to the collapse from conditional generation process into the unconditional process.
    To address this problem, we propose two simple but effective approaches from two perspectives.
    For sampling procedure, we introduce the entropy of predicted distribution as the measure of guidance vanishing level and propose an entropy-aware scaling method to adaptively recover the conditional semantic guidance. % for each generated sample. 
    For training stage, we propose the entropy-aware optimization objectives to alleviate the overconfident prediction for noisy data.
    % take uniform distribution as another supervision label and 
    % as another supervision for noisy data,
    % to alleviate the overconfident prediction from classifier, 
    % Finally, we constrain the entropy of predicted distribution provided from classifier.
    % and uniform distribution.
    % one-hot label is utilized to supervise the noisy data in previous work, ignoring the damaged semantic caused by noise
    % In addition to one-hot label, we take uniform distribution as another supervision for noisy data, constraining the divergence between predicted distribution of classifier and uniform distribution.
    On ImageNet1000 256$\times$256, with our proposed sampling scheme and trained classifier, the pretrained conditional and unconditional DDPM model can achieve 10.89\% (4.59 to 4.09) and 43.5\% (12 to 6.78) FID improvement respectively. 
    Code is available at \url{https://github.com/ZGCTroy/ED-DPM}.
    % achieve a FID (Fréchet Inception Distance) of 4.09 and sFID of 5.07, improving over the previous best FID of 4.59 and sFID of 5.25. 
    % Combined with our proposed schemes, the method based on unconditional DDPM architecture could achieve a 43.5\% relative improvement on FID.
    % We conduct experiments on ImageNet1000 and achieve state-of-the-art generation results for all resolutions, averagely with a 10\% relative improvement on FID (Fréchet Inception Distance).
    % Furthermore, our proposed methods can be easily extended into various architectures and sampling iteration methods without nearly any additional computation cost.
    % Based on unconditional DDPM architecture, our methods could achieve a 43.5\% relative improvement on FID.
    % outperforms previous state-of-the-art generative model, BigGAN-deep, which has not been achieved in previous work.
    % \dots
    \keywords{Denoising Diffusion probabilistic Model, Conditional Generation, Distribution Entropy, Gradient Vanishing}
    % Furthermore, our methods outperformed
    % BigGAN-deep on FID, based on only unconditional DDPM architecture.
    % Based on unconditional DDPM architecture, our methods achieved a 43.5\% relative improvement on FID.
    % , outperforming the results of BigGAN-deep.
    % FID of 6.78 and sFID of 6.56, compared with 
    % without conditional DDPM architecture 
    % , which is called \textbf{E}ntropy-\textbf{C}onstraint \textbf{T}raining scheme for classifier (ECT).
    % Experiments demonstrated that our proposed method outperformed existing methods on ImageNet benchmark and achieve state-of-the-art results in term of FID metric.
    % The classifier is trained under
    % build two Markov processes by introducing multiple time steps to generate samples, which has recently achieved remarkable performance in unconditional generation.
    % Furthermore, unconditonal DDPM can implement conditional generation flexibly by utilizing Bayesian theorem to decompose the conditional transition distribution into prior denoising distribution and likelihood distribution. 
    % The gradient of log likelihood density is computed by backwarding the pretrained classifier with desired condition label, providing conditional semantic guidance for DDPM.
\end{abstract}
% \begin{abstract}
% The abstract should summarize the contents of the paper. LNCS guidelines
% indicate it should be at least 70 and at most 150 words. It should be set in 9-point
% font size and should be inset 1.0~cm from the right and left margins.
% \dots
% \keywords{We would like to encourage you to list your keywords within
% the abstract section}
% \end{abstract}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/1-introduction.tex <==
\section{Introduction}
Conditional image generation, usually class conditional, aims to generate the specific class of high-quality images.
% that are close to the distribution in reality. 
% Generating a class-specific image is not just about being classified correctly
% In additional to class-aware generation results, fine-grained details such as texture, gloss, color, are also necessary.
% Different from Generative Adversial Networks (GAN) \cite{bigbigan,biggan} or Variational Autoencoder (VAE) \cite{vqvae2,nvae},
There are a lot of generative models which are able to make high-quality conditional generation based on joint-training scheme, like Generative Adversial Networks (GAN) \cite{bigbigan,biggan} or Variational Autoencoder (VAE) \cite{vqvae2,nvae}.
However, when the condition requirement is changed, the generative models will be retrained, which is very inconvenient.
\blfootnote{
$^{*}$Equal contribution \\
Preprint. Under review.}
\input{figure/first_img}

Denoising Diffusion Probabilistic Model (DDPM) \cite{ho2020denoising,nichol2021improved,song2020denoising} is a class of iterative generation models, which has made remarkable performance in unconditional image generation recently.
% Different from previous models, DDPM introduces multiple discrete time steps to model the non-parametric diffusion process from real data to prior noise and learns its reverse denoising process to generate samples via modeling the transition distribution.
The flexibility of DDPM  \cite{dhariwal2021diffusion,dickstein} is that it can be easily extended to conditional variants by introducing an independent noise-aware classifier.
% The Conditional diffusion generation models conditional transition distribution at each time step, 
% which can be decomposed into likelihood distribution and prior denoising distribution utilizing Bayes theorem. 
Recent researches modeled the prior denoising distribution by training an unconditional DDPM, following the training scheme of Denoising Score Matching \cite{vincent2011connection}, and computed likelihood score by backwarding the classifier gradient.
% trained an independent classifier under noisy data to model likelihood distribution.
% Specifically, the conditional guidance is provided by the gradient backwarding the pretrained classifier.
% The guidance term of classifier, which is computed by backwarding the classifier gradient, is utilized to provide conditional guidance
% \cite{dhariwal2021diffusion} derived the classifier gradient term from the likelihood distribution to rpovide
% applied this characteristic to
% the class-conditional generation task and trained an independent classifier under noisy data to provide conditional gradient guidance at each time step.
% Specifically, the prior denoising distribution is modeled by the unconditional DDPM, 
% following the training scheme of Denoising Score Matching \cite{vincent2011connection}, and the likelihood score is computed by backwarding the classifier gradient.
% The conditional generation process can be modeled by computing two distributions above at each time step.
% by introducing an independent classifier.
Dhariwal \etal~\cite{dhariwal2021diffusion} further proposed fixed scaling factor to improve the predicted probability of generated samples for DDPM, achieving superior performance than GAN on several image generation benchmarks.
% However, the constant scaling factor may not be conducive to conditional diffusion generation.

% However, the constant scaling factor for classifier guidance is inconsistent with the  variation law of effective gradient scale.
% we observed that the classifier only provided high-level semantic information.
In conditional generation process of DDPM, by backwarding the gradient of classification probability to image, the classifier provides high-level semantic information in the early stage of iterations, and gradually strengthens fine-grained features in the subsequent iterations, both of which are indispensable. 
However, there exists a huge gap between discriminating the class of a image and generating a specific class of image with fine-grained textures. As shown in Fig.\ref{fig:coverge}, the predicted distribution of the classifier for noisy images tends to quickly converge to the desired class distribution, which is one-hot distribution, leading to the early vanishing of conditional gradient guidance. This is because that the incompletely generated image, which is still a noisy image and lacks fine-grained features, can be easily classified in the middle of denoising process.
In this way, the image is considered to have been completely generated, and will no longer be guided by classifier gradient containing class information. As a result, the conditional generation process will degrade into an unconditional generation process in the later stage. 
 
% As a result, the generated samples will contain less condition-aware semantic information, leading to the degradation of conditional generation quality. 

% Specifically, the initial prior noise firstly evolved into noisy samples with high-level semantic information, guided by both the pretrained classifier and unconditional DDPM. Then, the samples are guided by unconditional DDPM completely without classifier, which could make generated samples lose the conditional fine-grained semantic guidance, as shown in Fig.\ref{fig:coverge} (b).
% The unconditional denoising process may 
% the classifier only provided class-level semantic guidance, which causes the lost of fine-grained semantic guidance.
% As shown in Fig\ref{fig:coverge}(2), 
% The gradient guidance prematurely vanished when the predicted probability approaches the maximum,
% leading to the loss of fine-grained semantic guidance.
% For example, when the predicted probability coverges to $0$, the gradient guidance vanishes.
% For example, as shown in Fig.\ref{fig:class_scale}, we compute the optimal scale factor for each class condition in ImageNet, from which it can be concluded that the effective scale varies greatly under different conditions.
% It motivated us to explore a dynamic scaling factor for classifier guidance at each time step.

% the effective scaling factor is dynamic, instead of static. 
% In addition, 
% we observe that the gradient tend to vanish prematurely.
% prematurely vanishing gradient
% In this paper, we consider 

% The reason can mainly be attributed to the effect of prior denoising score involved in conditional generation process.
% Specifically, when the predicted distribution approaches to one-hot distribution in the conditional sampling process, 
% the gradient guidance will vanish due to the sparsity of predicted distribution.
% which will be regarded as the noise information hidden in the sample 
% and conflicted with the denoising prior score.
% In detail, the gradient guidance will vanish
% However, the scaling factor for classifier guidance remains constant.
 

Therefore, our motivation is to enable the classifier to continuously give conditional guidance throughout the entire denoising process. We propose two simple but effective schemes from the procedure of sampling and the design of classifier training.

From the perspective of sampling procedure, we focus on how to detect the gradient vanishing and rescale the gradient to avoid the existence of gradient vanishing or recover the gradient when the vanishing does happen. 
We propose \textbf{E}ntropy-\textbf{D}riven conditional \textbf{S}ampling (EDS) method, which is able to adaptively measure the level of gradient vanishing and rescale the gradient guidance to a appropriate level. 
In design of training classifier, we propose \textbf{E}ntropy-\textbf{C}onstraint \textbf{T}raining (ECT), which will penalize the classifier when it gives a overconfident classification probability to a generated noisy image, thus constraining the classifier to provide more gentle guidance.

% Considering that the sparsity of predicted distribution tends to result in the weak gradient guidance, we take discrete uniform distribution, which is a more dense distribution, into consideration and constrain the divergence between the predicted distribution and uniform distribution, which is also the entropy-aware optimization loss.

% The conditional gradient guidance will be augmented adaptively for each sample at each time step, and the recovery level is controlled by the entropy-aware scaling.
% From the perspective of sampling / inference procedure, there exists stochasticity of transitions due to the characteristic of diffusion models \cite{choi2021ilvr}, which makes the vanishing time points various for generated samples.
% % Due to the randomness in the generation process for diffusion models,
% % the vanishing time points could be various for generated samples.
% Furthermore, the learning bias of classifier for each condition would make the the recovery levels for each condition differ from each other.
% We noticed that when the gradient guidance begins to vanish, the predicted distribution tends to converge to one-hot, which is a extremely sparse distribution.
% Considering that entropy can represent the sparsity of distribution,
% in this paper, we take this of predicted distribution as the measure of guidance vanishing level and propose a simple but effective entropy-aware scaling technology, which is named as \textbf{E}ntropy-\textbf{D}riven conditional \textbf{S}ampling (EDS).
% The conditional gradient guidance will be augmented adaptively for each sample at each time step, and the recovery level is controlled by the entropy-aware scaling.

% From the perspective of training, one-hot supervision pattern for noise-aware classifier could also contribute to the early vanishing guidance.
% Considering that the sparsity of predicted distribution tends to result in the weak gradient guidance, we take discrete uniform distribution, which is a more dense distribution, into consideration and constrain the divergence between the predicted distribution and uniform distribution, which is also the entropy-aware optimization loss.
% o approximate the noisy label.
% previous learning schemes forced the classifier to distinguish the noisy data under one-hot label supervision, 
% which directly takes the original label of the clean data as the supervision for noisy data.
% However, the label supervision for the noisy sample 
% The difficulty in estimating the noisy supervision label is that the transition kernel about the noisy label in diffusion process has no tractable form, and the prior distribution of noisy label can not be observed. 
% Considering that the noise added to sample will cover the semantic information randomly, in addition to clean label, we utilize discrete uniform distribution to approximate the noisy label.
% Specifically, we constrained the divergence between the predicted label distribution and uniform distribution, which is also the distribution entropy, by introducing an regularization term in the training stage of the classifier.


% Extensive experiments demonstrated the effectiveness of our proposed methods on ImageNet 256$\times$256 \cite{imagenet}.
% With our proposed training scheme,
% the performance has already achieve state-of-the-art performance in FID \cite{fid} and IS \cite{noteoninceptionscore}.
% Combined with the regularization term designed in the training stage of the guiding classifier, the conditional generation performance will be further improved.
% Furthermore, we perform the ablation studies to verify the performance contribution of each method.
Our contributions can be summarized as follows:
\begin{itemize}
    \item[$\bullet$] We are the first to discover the problem of vanishing gradient guidance for ddpm-based conditional generation methods, and point out that category information guidance should be continuously provided throughout the entire generation process.
    \item[$\bullet$]  We propose EDS to alleviate the vanishing guidance by dynamically measuring and rescaling gradient guidance.
    % To alleviate the overconfident prediction for noisy data, we propose ECT, entropy-aware
    At the training stage of classifier, for alleviating the vanishing gradient caused by one-hot label supervision, we utilize discrete uniform distribution to build an entropy-aware optimization term, which is \textbf{E}ntropy-\textbf{C}onstraint \textbf{T}raining scheme (ECT).
	\item[$\bullet$] We conduct experiments on ImageNet1000 and achieve state-of-the-art FID (Fréchet Inception Distance) results at various resolutions. On ImageNet1000 256$\times$256, with our proposed sampling scheme and trained classifier, the pretrained conditional and unconditional DDPM model can achieve 10.89\% (4.59 to 4.09) and 43.5\% (12 to 6.78) FID (Fréchet Inception Distance) improvement respectively. 
% 	Combined with our schemes, the method based on unconditional DDPM architecture could achieve a 43.5\% relative improvement on FID.
% 	Furthermore, our methods improved FID from 12 to 6.78, achieving a nearly 40\% relative gain, based on unconditional DDPM architecture.
% 	.benchmark state-of-the-art performance in ImageNet  \cite{imagenet} benchmark in term of FID metric, outperforming existing methods. 
\end{itemize}



==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/2-related_work.tex <==
\section{Related Work}
\subsection{Denoising Diffusion Probabilistic Model}
Denoising diffusion probabilistic models (DDPM) is the latest generation model which achieve superior generation performance than traditional generative models like Generative Adversial Networks (GAN) \cite{gan,bigbigan,biggan}, Variational Autoencoders (VAE) \cite{nvae,vqvae,vqvae2} on several benchmarks about unconditional generation.
Its key idea is to model the diffusion process based on total $T$ time steps, which adds noise gradually to the clean data, and its reverse process, which denoises the white noise into the clean sample.
Accordingly, its diffusion process is modeled as a fixed Markov Chain and its transition kernel is formulated as:
\begin{equation}\label{eq:rw_forward}
q(\bx_{t}|\bx_{t-1}):=\mathcal{N}(\bx_{t};\sqrt{1-\beta _{t}}\bx_{t-1},\beta _{t}\mathbf{I}),
\end{equation} 
where $\beta_1,...,\beta_T$ are the fixed variance parameters, which are not learnable.
According to the transition kernel above, when the clean data $\bx_0$ is given, the noisy data $\bx_t$ can be sampled with a close-formed distribution:
\begin{equation}\label{eq:sample_diffusion}
q(\bx_{t}|\bx_{0})=\mathcal{N}(\bx_{t};\sqrt{\overline{\alpha}_{t}}\bx_{0},(1-\overline{\alpha}_{t})\mathbf{I}),
\end{equation}
where $\alpha_t=1-\beta_t$ and $\bar \alpha_t=\prod_{s=1}^t \alpha_s$.
When $t$ is close to $T$, $x_T$ can be approximated as a Gaussian distribution.

Given a prior diffusion process, DDPM aims to model its reverse process to sample from the data distribution.
% However, the reverse of the forward process $q(\bx_{t-1}|\bx_t)$ has no tractable solution.
The optimization objective of the reverse transition can be derived from a variational bound \cite{kingma2014auto}.
Thus, DDPM introduced the variational solution \cite{kingma2014auto} and assumed that its reverse transition kernel also subjects to Gaussian distribution, which is the same as the diffusion process.
In this way, the generation process parameterized the mean of the Gaussian transition distribution and fixed its variance as follow:
\begin{equation}\label{eq:reverse}
\begin{split}
p_{\theta}(\bx_{t-1}|\bx_{t})=\mathcal{N}(\bx_{t-1};\mu_{\theta}(\bx_t),{\sigma}_t^2\mathbf{I}) 
\\
\mu_{\theta}(\bx_t)=\frac{1}{\sqrt{\alpha_{t}}}(\bx_{t}-\frac{1-\alpha _{t}}{\sqrt{1-\bar {\alpha}_{t}}}\bepsilon_{\theta }(\bx_{t})),
\end{split}
\end{equation}
% For optimizing the variational bound,
% the predicted mean $\mu_{\theta}(\bx_t)$ is parameterized as:
% \begin{equation}\label{eq:sampling}
% \mu_{\theta}(\bx_t)=\frac{1}{\sqrt{\alpha_{t}}}(\bx_{t}-\frac{1-\alpha _{t}}{\sqrt{1-\bar {\alpha}_{t}}}\bepsilon_{\theta }(\bx_{t})),
% \end{equation}
where $\bepsilon_{\theta }(\bx_{t})$ is a noise estimator modeled by a neural network.
The variance is designed as the hyperparameters for training diffusion models.

Recently, there were some researches \cite{scorematching,sde,ddim,dhariwal2021diffusion} which indicated that the noise estimator can be regarded as an approximation of score function so that the sampling process is equivalent to solving a stochastic differential equation.
% \begin{equation}\label{eq:score_equal}
% \nabla_{\bx_t} \log p_{\theta}(\bx_t) = - \frac{1}{\sqrt{1- \bar \alpha_t}} \bepsilon_{\theta}(\bx_t).
% \end{equation}
Based on above, Song.et \cite{ddim} proposed an effective sampling process that shares the same training objectives as DDPM and its corresponding denoising process, which is also the iteration solution to solve the stochastic differential equation, is designed as followed:
\begin{equation}\label{eq:ddim_sample}
\bx_{t-1}=\sqrt{\alpha_{t-1}}f_{\theta}(\bx_t, t) + \sqrt{1-\alpha_{t-1}-\sigma_t^2} \epsilon_{\theta}(\bx_t) + \sigma_t^2 \mathbf{\bz},
\end{equation}
where $f_{\theta}(\bx_t,t)$ is the prediction of clean data $x_0$ when the noisy data $\bx_t$ is observed and noise prediction $\bepsilon_{\theta}(\bx_t)$ is given.
The specific form of $f_{\theta}(\bx_t,t)$ can be expressed as:
\begin{equation}\label{eq:ddim_predx0}
f_{\theta}(\bx_t, t)=\frac{\bx_t-\sqrt{1-\alpha_t}\bepsilon_{\theta}(\bx_t)}{\sqrt{\alpha_t}},
\end{equation}
When the variance $\sigma_t$ is set to 0, the sampling process becomes deterministic.
At the same time, the non-Markovian diffusion process \cite{ddim} allows that the generation quality remains unchanged within fewer denoising steps, which is called DDIM sampling process.
% In \cite{ddim}, DDIM can be regarded as a Euler method to solve ODE by rearranging the sampling formula as follows:
% \begin{align}\label{eq:ddim_sample_rearrage}
% \begin{split}
% \bx_{t-1} - \bx_t=\sqrt{\alpha_{t-1}}[(\sqrt{1/\alpha_t}-\sqrt{1/\alpha_{t-1}})\bx_t \\
% + (\sqrt{1/\alpha_{t-1} - 1}-\sqrt{1/\alpha_t - 1})\bepsilon_{\theta}(\bx_t,t)].
% \end{split}
% \end{align}


\subsection{Conditional Image Generation}
Conditional image generation aims to generate samples with desired condition information.
The condition can be extended to multi-modal information, such as class \cite{cgan,vqvae,vqvae2,xiao2021conditional}, text \cite{xia2021tedigan,ramesh2021zero,wang2021cycleconsistent}, and low-resolution image \cite{bulat2018learn}.
Most previous work modeled this by the joint training scheme with both condition and random noise, utilizing generative models like GAN or VAE.
% The most research utilized GAN due to its remarkable generation quality
% such as.....
% and make conditional generation by the joint training scheme of both condition and 
% conditional GAN, such
% as ....

Considering that Denoising Diffusion Probabilistic Model (DDPM) has made remarkable progress in recent years \cite{ddim,kingma2021variational,ddimdistill,huang2021variational,de2021diffusion,song2021maximum,nachmani2021non,nie2021controllable}, there raised many researches \cite{dhariwal2021diffusion,diffwave,choi2021ilvr,sasaki2021unit,sinha2021d2c,liu2021diffsinger,lyu2021conditional} which applied DDPM to conditional generation.
Due to the ideal theoretical properties of DDPM, it can be extended flexibly to conditional variants utilizing Bayes theorem without retraining, which is similar with score-based generative models \cite{scorematching,sde,meng2021sdedit}.
In this paper, we focus on the class-conditional generation task,
in which the condition is represented by a class discrete distribution, and design a more effective sampling and training scheme to improve the generation quality for DDPM, further exploring its potential in image generation aspects.
% Recent researches experimented on ImageNet256$\times$256.
% The recent success of DDPM inspired \cite{ddpm} to explore its potential in conditional generation, making conditonal DDPM outperform BigGAN-deep in term of FID metric.
% The recent state-of-the-art method utilize the property of DDPM
% and extended it to conditional models by bayes theorem,
% outperforming BigGAN-deep in term of FID metric.




==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/3-proposed_methods.tex <==
% \usepackage{xr}
% \externaldocument{2-related_work.tex}

\section{Proposed Methods}
% implicit label modeling
% whole scheme
% The conditional generation process for the diffusion models 
We start by introducing the conditional generation process for diffusion models with classifier guidance (Sect.(\ref{md:cdg})).
% Then, we point out that the vanishing conditional gradient can be partly attributed to the sparse label supervision for noise-aware classifier, and the discrepancy between discriminative and generative patterns, and the sparse label supervision.
For ease of description, we will firstly introduce our dynamic scaling technology to recover gradient guidance adaptively in the sampling process and its motivation (Sect.(\ref{md:eds})).
% motivated by the fact that there exists randomness in the predicted distribution of the guided classifier.
Then, we describe the entropy-aware optimization loss for alleviating vanishing conditional guidance from training perspective (Sect.(\ref{md:ect})), utilizing the uniform distribution, which is a more dense distribution.
% Finally, we summary the overall training and sampling schemes for conditional diffusion generation (Sect.(\ref{md:overall})).


\subsection{Conditional Diffusion Generation}
\label{md:cdg}

% \subsubsection{Overall Training and Sampling Scheme}
% \label{md:overall}
% In this section, we summary our algorithm pipeline.
% Our target is to utilize the unconditional pretrained diffusion model $\epsilon_{\theta}(\bx_t,t)$ to make conditional generation.
% Firstly, we follow \cite{dickstein,sde} and utilize Bayesian theorem to decompose the target term into two independent terms in  Eq.\eqref{eq:cond_gaussian_format}.
% In this way, we only need to train an independent classifier under noisy data and backward the gradient to model the gradient field.

% When training the classifier, in addition to normal likelihood loss term,
% we propose a simple but effective regularization term, constraining the divergence between predicted distribution and uniform distribution.
% The training detail is shown in Algorithm.\ref{alg:entropy_constraint_train}.

% In the sampling process, considering the vanishing gradient from guiding classifier $\phi$,
% we rescale the gradient by the proposed entropy-aware factor,
% alleviating the level of vanishing guidance dynamically.
% The details of sampling scheme is shown in Algorithm.\ref{alg:entropy_driven_ddpm} and Algorithm.\ref{alg:entropy_driven_ddim}.



% introduce the class-conditional generation task and 
% claim our model target p(y|x)&\nabla p(y|x)
% For diffusion models, conditional generation can be implemented by introducing an independent classifier.
The goal of conditional image generation is to model probability density $p(\bx|\by)$.
To be specific, in class-conditional image generation, $\by$ represents the desired class label, which tends to be one-hot distribution, and $\bx$ represents the image sample.
% For diffusion models, it can be extended to conditional models 
% by introducing the gradient guidance from an independently trained classifier.
% In this section, we claim that our propose is to model $p(x_0|c)$, in which $x_0$ means the clean image.
%   (We start with the conditional sampling for a diffusion model.
For diffusion models, it can be implemented by introducing an independent classifier, as shown in Fig.\ref{fig:pipeline}.

% instead of modeling $p(\bx|\by)$, 
Specifically, the goal is converted into modeling the conditional transition distribution $p(\bx_{t-1}|\bx_{t},\by)$, derived from Markov chain sampling scheme:
% For this purpose, we can sample images from the conditional distribution $p(x_0|c)$):
\begin{equation}\label{eq:cond_markov}
\begin{split}
p_{\varphi}(\bx_{0}|\by)&=\int_{}^{}p_{\varphi}(\bx_{0:T}|\by)d\bx_{1:T}, \\
p_{\varphi}(\bx_{0:T}|\by)&=p(\bx_{T})\prod_{t=1}^T p_{\varphi}(\bx_{t-1}|\bx_{t},\by),
\end{split}
\end{equation}
where $\varphi$ represents the model and $T$ is the total length of Markov chain, which tends to be large.
% Diffusion models connect prior distribution to the real data distribution by adding noise perturbation.
% copy from NIPS 2021
Then, we decompose the conditional transition distribution into two independent terms:
% \cite{dickstein,dhariwal2021diffusion} demonstrated  that the conditional transition distribution can be decomposed into two independent terms:
\begin{align}\label{eq:cond_kernel_decompose}
\begin{split}
p_{\varphi}(\bx_{t-1}|\bx_t,\by)=Zp_{\theta}(\bx_{t-1}|\bx_{t})p_{\phi}(\by|\bx_t),
\end{split}
\end{align}
% \theta, \phi
where $Z$ is a normalizing constant independent from $\bx_{t-1}$ and $\varphi$ can be seen as the combination of models $\theta$ and $\phi$,
which is proven theoretically \cite{dickstein,dhariwal2021diffusion}.
Furthermore, the log density of Eq.\eqref{eq:cond_kernel_decompose} can be approximated as a Gaussian distribution \cite{dhariwal2021diffusion}:
\begin{equation}\label{eq:cond_gaussian_format}
\begin{split}
&\log (p_{\varphi}(\bx_{t-1}|\bx_t,\by)) \approx \log p(\bz) + \log Z \\
\bz &\sim \mathcal{N}(\frac{1}{\sqrt{\alpha_{t}}}(\bx_{t}-\frac{1-\alpha _{t}}{\sqrt{1-\bar {\alpha}_{t}}}\bepsilon_{\theta }(\bx_{t})) + \sigma^2_t \bg,{\sigma^2_t} \mathbf{I}),
\end{split}
\end{equation}
where $\bg=s\nabla_{\bx_t} \log p_{\phi}(\by|\bx_t)$ and $s$ is the gradient scale.
$\bg$ can be derived by backwarding the gradient of a pretrained classifier about noisy data $\bx_t$.
Usually, $s$ is set to a constant \cite{dhariwal2021diffusion} to improve the predicted probability.
% a constant scale and introduced \cite{dhariwal2021diffusion} to improve the predicted probability.
$\bepsilon_{\theta }(\bx_{t})$ is the pretrained noise estimator for diffusion models and 
$\sigma^2_t$ is the hyperparameters for unconditional DDPM to control the variance.
% $\mu_{\theta}(\bx_t)$ is the same with that in Eq.\eqref{eq:reverse}.

% from which 
% We notice that $p_{\theta}(x_{t-1}|x_{t})$ can be modeled by unconditional denoising process.
% To this end, we use a score-based conditioning trick adapted from xxx(), which leverages the connection between diffusion models and score matching.
% In particular, if we have a model $\epsilon_{\theta}(x_t)$ that predicts the noise added to a sample, then this can be used to derive a score function:
% \begin{align}\label{eq:scorenet}
% \begin{split}
% \nabla_{x_t} \log p_{\theta}(x_t)=-\frac{1}{\sqrt{1-\bar \alpha_t}}\epsilon_{\theta}(x_t)
% \end{split}
% \end{align}
% We can now substitute this into the score function for $p(x_t)p(y|x_t)$:
% \begin{align}\label{eq:condscore}
% \begin{split}
% \nabla_{x_t} \log (p(y|x_t))=\nabla_{x_t} \log p_{\theta}(x_t) +\nabla_{x_t} \log p_{\phi}(y|x_t) \\
% =-\frac{1}{\sqrt{1-\bar{\alpha}_t}} \epsilon_{\theta}(x_t) +\nabla_{x_t} \log p_{\phi}(y|x_t)
% \end{split}
% \end{align}
% Finally, we can define a new epsilon predictionˆ(xt)which corresponds to the score of the joint distribution:
% We can get conditional noise prediction format as follows:
% \begin{align}\label{eq:condeps}
% \begin{split}
% \tilde \epsilon(x_t) = \epsilon_{\theta}(x_t) - \sqrt{1 - \bar{\alpha}_t} \nabla_{x_t} \log p_{\phi}(y|x_t)
% \end{split}
% \end{align}
% After training the noise-based classifier, we can get the $ \nabla_{x_t} p_{\phi}(y|x_t) $ through gradient backward.
%   
% claim the existing problem.
% the problem exists in the classifier mistake due to the stochastic noise involved in the training scheme.

% Recently, there exists another generative method via a class of non-Markovian processes \cite{ddim} for diffusion models, which is called DDIM (Eq.(\ref{eq:ddim_sample})).
% % We will show that our scaling technology can be easily extended to this class of iteration approach.
% Specifically, when a noise approximator $\bepsilon_{\theta}(\bx_t)$ is pretrained, it can be utilizied to model the score function, which is involved in the generative stochastic differential equation \cite{ddim,sde}:
% \begin{equation}\label{eq:score_function}
% \begin{split}
% \nabla_{\bx_t} \log p_{\theta}(\bx_t)= 
% -\frac{1}{\sqrt{1-\bar \alpha_t}} \bepsilon_{\theta}(\bx_t).
% \end{split}
% \end{equation}

% With score function modeled above, the goal of conditional generation can be converted into modeling $\nabla_{\bx_t} \log p_{\varphi}(\bx_t|\by)$.
% Then, we decompose the conditional score utilizing Bayesian theorem as followed:
% % Utilizing Bayesian theorem, the conditional score can be further decomposed as followed:
% \begin{equation}\label{eq:bayes_score}
% \begin{split}
% \nabla_{\bx_t} \log p_{\varphi}(\bx_t|\by)&= 
% \nabla_{\bx_t} \log p_{\theta}(\bx_t)
% +
% \bg
% -
% \nabla_{\bx_t} \log p(\by)
% \end{split}
% \end{equation}
% where $\bg = \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t)$.
% In order to improve the predicted probability of desired classes for final generated samples,
% an invariant scaling factor $s$ is proposed \cite{dhariwal2021diffusion} at each time step for Eq.\eqref{eq:bayes_score} and Eq.\eqref{eq:cond_gaussian_format}:
% % to augment the gradient guidance:
% \begin{equation}\label{eq:cond_gaussian_scale}
% \begin{split}
% \bg = s\nabla_{\bx_t} \log p_{\phi}(\by|\bx_t).
% % z \sim \mathcal{N}(\mu_{\theta}(x_t)+s\sigma_t g,{\sigma^2_t} \mathbf{I}),
% \end{split}
% \end{equation}

In this way, unconditional diffusion models with parameterized noise estimator $\bepsilon_{\theta}$ can be extended to conditional generative models by introducing the condition-aware guidance $\nabla_{\bx_t} \log p_{\phi}(\by|\bx_t)$, 
% which is derived from an independently trained classifier under noisy data $\bx_t$, into the generation process, 
as shown in Fig.\ref{fig:pipeline}.
Specifically, we start with the prior noise $\bx_T \sim \mathcal{N}(0,\bI)$, and utilize DDPM-based (Eq.\eqref{eq:cond_gaussian_format}) sampler to make transition iteratively to generate the samples conditioned on desired class $\by$.
The sampler can also be extended into DDIM iteration method (Eq.\eqref{eq:reverse}). The extension details for conditional process with classifier guidance can refer to Dhariwal \etal \cite{sde,dhariwal2021diffusion}.
% as shown in Fig.\ref{fig:pipeline}.
% {eq:reverse}

\input{figure/pipeline}
\subsection{Entropy-driven Conditional Sampling}
\label{md:eds}

\input{figure/vanishing_point_hist}
During the conditional generation process, we observe that the guidance provided from noise-aware classifier tends to vanish prematurely,
% Normally, when the sample converges into sparse predicted distribution, its conditional probability will achieve to 1, in which state the gradient guidance has been weak, while the sample still lacks semantic details.
which could be attributed to the discrepancy between generative pattern and discriminative pattern.
For example, the noisy samples with high-level semantic information, such as contour or the color, may be guided iteratively by the classifier with nearly one-hot distribution,
in which situation the gradient guidance tends to be weak or vanish, while the samples still lack the condition-aware semantic details. 
% When the predicted distribution approaches one-hot form, the gradient of classifier tends to vanish.
% Specifically, the classifier may discriminate noisy sample by only high-level semantic information, such as contour or color, and predict a nearly one-hot distribution, leading to the early vanishing of gradient guidance.
% may predicted the noisy sample with nearly one-hot distribution. For example, the classifier 
% due to the class-aware semantic information hidden in the noisy sample.
In this way, the condition-aware textures of generated samples are guided by unconditional denoising process (Eq.\eqref{eq:reverse}).
% because the noise hidden in sample 
% the predicted distribution of the classifier for generated images tends to be quickly converged to the desired class distribution, which is one-hot distribution, leading to the early vanishing of conditional gradient guidance.
% in the training stage of the guiding classifier,
% One-Hot label distribution is utilized to supervise the noisy sample in all different diffusion level (Eq.\eqref{eq:sample_diffusion}),
% which could cause the different vanishing level of the gradient guidance due to the extreme sparsity of supervision label.
% To be specific, when the noise level is low and $t$ approaches $0$, the noisy samples 
% $\bx_t$ maintain most of discriminative semantics,
% so that the predicted distribution $p(\tilde \by|\bx_t)$ tends to be sharper
% and the gradient guidance may vanish.
% In the opposite, when the noise level is high enough and $t$ approaches $T$, the noisy sample $\bx_t$ is close the the white Gaussian noise, 
% which contains no semantic information and the gradient guidance tends to be augmented.
% The regular of gradient norm is shown as Fig.\ref{fig:gradnorm_and_p}.
% \input{fig/compare_gradnorm_and_p}


% \begin{figure}[t!]
%     \begin{center}
%     \includegraphics[width=1.0\textwidth]{figure/vanishing_point_hist.jpg}
%     \caption{\textbf{The statistical distribution about initial time points of vanishing gradient.} We randomly sample about 5000 samples and set a norm threshold to select the initial time step of the vanishing gradient.
%     We can observe that most samples can not be guided by classifier gradient prematurely, and the time steps of vanishing varies greatly between each other.}
%     \end{center}\label{fig:vanishing_hist}
%     \vskip -0.2in
% \end{figure}

An intuitive solution is to manually select a time step during the sampling process, after which the semantic details tend to vanish in most instances, and rescale the conditional gradient by an empirical constant after the selected time step.
However, since the stochasticity in the generation process of diffusion models \cite{choi2021ilvr},
the denoising trajectories for generated samples would differ from each other. 
It will lead to the various initial vanishing points, as shown in Fig.\ref{fig:vanishing_hist}.
At the same time, considering the learning bias of classifier for different conditional classes, the level of recovery factor for each class may also differ.
% such a practice is computationally expensive especially for large systems, e.g., proteins, and is sometimes unnecessary,
% The experiment results can be seen as .....
In summary, the effective scaling factor can be related to the current time step, the class condition, and the stochasticity of generation process.
The experiment design and results about more intuitive approaches can be seen in Sect.\ref{exp:eds_ab}.
% Furthermore, the optimization objective for effective scale function is hard to design, which leads to the difficulty of manually designing.

Motivated from above, we propose an dynamic scaling technology for the conditional diffusion generation to recover the semantic details adaptively for each sample.
We noticed that, when time step is close to $T$, the predicted distribution tends to be dense, which can be nearly approximated as uniform distribution.
The reason is that the noisy data derived from Eq.\eqref{eq:rw_forward} can be approximated as random noise, $\mathcal{N}(0,\bI)$,
in which state the gradient guidance is obvious.
As time step declines to $0$ inversely, the noise hidden in sample will be removed gradually and the predicted distribution tends to be close to one-hot, in which case the classifier gradient is invalid to provide semantic details for generation.
% When time step $T$ declines to $0$,
% the predicted distribution will become more and more sparse.
Statistically, entropy can represent the sparsity of the predicted distribution, inspiring us to take it into consideration:
\begin{equation}\label{eq:condentropy}
\begin{split}
\mathcal{H}(p_{\phi}(\tilde \by|\bx_t)) &= - \E_{\tilde \by|\bx_t} \log p_{\phi}(\tilde \by|x_t) \\
 &= - \sum_{i=1}^{|Y|} p_{\phi}(\tilde \by_i|\bx_t) \log p_{\phi}(\tilde \by_i|\bx_t),
\end{split}
\end{equation}
where $p_{\phi}(\tilde \by|\bx_t)$ represents the predicted distribution from classifier and $Y$ represents the set of all class conditions.
\input{algorithm/entropy-sampling}

In this paper, we utilize $\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))$ to adaptively fit various gradient vanishing time step.
Furthermore, the entropy $\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))$ can also capture bias caused by different conditions, due to its sample-aware rescaling effect.
% To be specific, for predicted condition distribution $p_{\theta}(\by|\bx_t)$ at time step $t$, we take its entropy into consideration and propose an entropy-aware scaling method.
% We take the entropy of the predicted distribution into consideration,
% When the predicted distribution approaches one-hot distribution by backwarding the classifier gradient iteratively (Eq.\eqref{eq:cond_gaussian_format}), 
% the entropy will decline to $0$.
% when the entropy approaches $0$, the guiding gradient in Eq.\eqref{eq:cond_gaussian_scale} decays and becomes sparse.
% In this paper, we utilize the entropy to construct the scaling factor for conditional semantic recovery:
% sparsity of predicted distribution:
% Specifically, the entropy of class-conditional predicted distribution $p(y|x_t)$ is formulated as:
% which can be formulated as:
Thus, when we sample from a pretrained noise estimator $\bepsilon_{\theta}$ in Eq.(\eqref{eq:cond_gaussian_format}) conditionally, 
we reformulate the gradient term $\bg$ as following, which is shown in Fig.\ref{fig:pipeline}:
% the entropy-driven sampling scheme can be formulated as:
\begin{equation}\label{eq:condsample}
\begin{split}
\bg' &= s(x_t, \phi) * \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t), \\
s(x_t, \phi) &= \gamma * \frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))}
% \bx_{t-1} &= \mu_{\theta}(\bx_t) + \sigma^2_t \bg' + \sigma_t \bepsilon,
\end{split}
\end{equation}
where 
% $\bepsilon$ subjects to $\mathcal{N}(\bzero,\mathbf{I})$,
% $\tilde \by$ represents the predicted class distribution, and 
$\bgamma$ is a hyper-parameter to balance the guiding gradient and entropy-aware scaling factor $s(\bx_t,\phi)$.
% $\mu_{\theta}(\bx_t)$ can be derived from pretrained unconditional DDPM in Eq.\eqref{eq:sampling}.
In order to maintain the numerical range, we renormalize the entropy by its theoretical upper bound $\mathcal{H}(\mathcal{U}(\tilde \by))$, where $\mathcal{U}(\tilde \by)$ represents the uniform distribution of class variable, so that the gradients are almost not rescaled when $t$ is close to $T$.
% Compared with previous conditional sampling scheme \cite{dhariwal2021diffusion}, our scheme 
% As time step $t$ decreases, the entropy-aware scaling will 

% In additional to sampling method based on Markov process(Eq.(\ref{eq:cond_markov})), recently there exists another iteration approach depending on the non-markov process.
% Our scaling technology can be extended into the conditional score nearly without any additional computation cost:
% \begin{equation}\label{eq:bayes_score}
% \begin{split}
% \nabla_{\bx_t} \log p_{\varphi}(\bx_t|\by)
% &= -\frac{1}{\sqrt{1-\bar \alpha_t}} \bepsilon_{\theta}(\bx_t) +
% \gamma * \frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t)
% \end{split}
% \end{equation}


% For the DDIM sampling method (Eq.\eqref{eq:score_equal}), which can reduce number of the iteration steps and accelerate the generation process, our sampling scheme replaced the noise approximator with the followling:
% \begin{equation}\label{eq:cond_score}
% \begin{split}
% \hbepsilon = \bepsilon_{\theta}(\bx_t) - \gamma * \frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t)
% \end{split}
% \end{equation}




\subsection{Training Noise-aware Classifier with Entropy Constraint}
\label{md:ect}
% Entropy-driven Sampling scheme can rescale the guiding gradient and alleviate the weak guidance for semantic details adaptively.
% However, this sampling can only adjust the updating step with scale with unchanged gradient direction.
From the training perspective, the vanishing gradient can be partly attributed to the label supervision pattern for noise-aware classifier.
Since one-hot distribution is very sparse and is utilized to supervise the noisy data, the predicted distributions are inclined to converge to one-hot under noisy samples in the sampling process, so that the gradient guidances are too weak to generate condition-aware semantic details at sampling stage.
% the vanishing gradient from noise-aware classifier at sampling stage.

% Different from $\bx_t$, which can be sampled according to Eq.\eqref{eq:sample_diffusion}, the probability density of $\by_t$ has no closed form solution.
% In previous work, they assume that the noise in label $y_t$ is small enough and set $\by_t \approx \by_0$, where $\by_0$ represents the supervision label assigned to clean sample $\bx_0$, to make the training of guiding classifier feasible.

% However, $\by_t$ can not be regard as $\by$ in most time, because the noise in diffusion process will cover the semantic information hidden in the sample.
% For example, when the noise added in the image data is close to the Gaussian noise,
% the semantic information hidden in image is lost mostly so that the class label can not be regarded as the same as the original $\by_0$.
% Thus, the prior conditional diffusion in Eq.\eqref{eq:cond_markov} is rewritten as:
% \begin{equation}\label{eq:cond_modified_markov}
% \begin{split}
% p_{\varphi}(x_{0:T}|y_t)&=p(x_{T})\prod_{t=1}^T p_{\varphi}(x_{t-1}|x_{t},y_t).
% \end{split}
% \end{equation}
% The intuitive approach is to follow the diffusion process of noisy sample $\bx_t$ and formulate the label diffusion process by Gaussian transition kernel, which is formulated as followed:
% \begin{align}\label{eq:diffusion_y}
% \begin{split}
% p_{\sigma}(\by_t|\by_0)=\frac{1}{(2\pi)^{1/2}\sigma} e^{-\frac{1}{2\sigma^2}||\by_t - \by_0||^2},
% \end{split}
% \end{align}
% % smoothing  kernel  or  noise  model:
% % sampled  from  isotropic  Gaussian
% where $\sigma$ represents the variance.
% However, this is an ideal assumption.
% In fact, the class label represents the conditional semantic information hidden in the sample and its regular of evolution may be extremely different from that of the noisy sample.
% Different from previous work, our method is proposed from the training perspective.

% \input{algorithm/entropy-training}

% In addition to label supervision $y_0$,
Specifically, given the dataset $(\bx_0, \by) \sim \mathbb{D}$ and a prior diffusion process (Eq.\eqref{eq:rw_forward}), the classifier will be trained under noisy data ${\bx_t}$ to build the gradient field in Eq.\eqref{eq:cond_gaussian_format} of each time step.
To alleviate the weak guidance caused by the sparsity, we utilize discrete uniform distribution, which is a dense distribution and has maximum entropy, as a perturbing distribution and introduce the optimization term at the training stage of the classifier to constrain the predicted distribution from the classifier as followed:
\begin{align}\label{eq:noisy_y}
\begin{split}
\mathcal{L}_{ECT}(\bx_t, \by) &= D_{KL}(p_{\phi}(\tilde \by|\bx_t) || \mathcal{U}(\tilde \by)) \\
&= \E_{\tilde \by|\bx_t} \log p_{\phi}(\tilde \by|\bx_t) - \E_{\tilde \by|\bx_t} \log \mathcal{U}(\tilde \by) 
\\
&= -\mathcal{H}(p_{\phi}(\tilde \by|\bx_t)) + \mathbf{C},
\end{split}
\end{align}
where $\mathbf{C}$ is a constant term independent from the parameter $\phi$.
This loss term is equivalent to maximizing entropy of the predicted distribution $p(\tilde \by|\bx_t)$.
% It can be complementary with entropy-driven sampling scheme, which can be seen from Sect...
The whole training loss of guiding classifier is composed of the normal cross-entropy loss and entropy constraint training loss (ECT), which is formally given by:
\begin{equation}\label{eq:noisy_training_loss}
\begin{split}
\mathcal{L}_{tot}(\bx_t,\by)=\mathcal{L}_{CE}(\bx_t,\by) + \eta  \mathcal{L}_{ECT}(\bx_t,\by),
\end{split}
\end{equation}
where $\eta$ is a hyper-parameter to adjust the divergence about
predicted label distribution and the uniform distribution.
\input{algorithm/entropy-training}

Different from Entropy-driven Sampling, the proposed training scheme tries to alleviate the vanishing guidance by adjusting the gradient direction in sampling process, instead of the gradient scale.
Thus, entropy-constrain training scheme can be complementary with entropy-driven sampling.
% which is shown in Sect.\ref{exp:overall_ab}.
% The detailed algorithm is shown in Algorithm.\ref{alg:entropy_constraint_train}.

% Compared with Entropy-driven Sampling, which rescales the gradient guidance adaptively, the entropy-constrain training tries to alleviate the weak guidance from the gradient direction.
% The weak gradient guidance is achieed when the predicted distribution is close to one-hot, ovverconfident distribution.
% The training scheme provides more dense predicted distribution, so that the gradient can be more dense.


% \subsection{Overall Training and Sampling Scheme}
% \label{md:overall}
% In this section, we summary our algorithm pipeline.
% Our target is to utilize the unconditional pretrained diffusion model $\epsilon_{\theta}(\bx_t)$ to make conditional generation.
% Firstly, we utilize Bayesian theorem \cite{dickstein,sde} to decompose the target term into two independent terms.
% In this way, we only need to train an independent classifier under noisy data and backward the gradient to model the gradient field.

% When training the classifier, 
% In addition to normal likelihood loss term, we propose a simple but effective regularization term, constraining the divergence between predicted distribution and uniform distribution.
% The training details are shown in Algorithm.\ref{alg:entropy_constraint_train}.

% In the sampling process, considering the vanishing semantic guidances from guiding classifier $\phi$, we rescale the gradient by the proposed entropy-aware factor, alleviating vanishing level adaptively, as shown in Fig.\ref{fig:pipeline}.
% Our proposed schemes can be easily extended into different iteration sampling methods, such as ddpm or ddim, without nearly any additional computation cost.
% The details of sampling scheme are shown in Algorithm.\ref{alg:entropy_driven_ddpm}.




==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/4-experiments.tex <==


\section{Experiments}
In this section, we present experiments to verify the effectiveness and motivation of our proposed schemes. More visualization of generated samples and ablation experiments about hyperparameters can be found in supplementary materials.
% Firstly, we provide the benchmark details, evaluation metrics, and the experimental configurations.
% Next, we evaluate the proposed methods quantitatively against the state-of-the-art results.
% Lastly, we conduct ablation experiments to analyse the impacts
% of our training and sampling scheme separately.

\subsection{Experiment Setup}
% \vspace{-1pt}
\paragraph{\textbf{Dataset}}
% \textbf{Dataset.}
We perform our experiments mainly on ImageNet dataset \cite{imagenet} at 256$\times$256 resolutions.
ImageNet contains 14,197,122 images with 1000 classes in total, which is a very challenging benchmark for conditional image generation.
% The experiments based on 128$\times$128, 64$\times$64 can be found in supplementary materials.
% which is a variant of FID and more sensitive to the consistent image distribution with high-level structures.

% To further verify the effectiveness of our proposed methods, we extend them to the settin,s of  different solutions, such as 64$\times$64 and 128$\times$128.
% Most widely used indicators
\vspace{-2pt}
\paragraph{\textbf{Implementation Details.}}
% We verify the effectiveness of our proposed training and sampling schemes on the same 
For verifying the effect of proposed schemes, we apply the neural network architecture, ablated diffusion model (ADM), proposed by Dhariwal.et al \cite{dhariwal2021diffusion}. 
ADM is mainly based on the UNet, with increased depth versus width, the number of attention heads, and rescaling residual connections with $\frac{1}{\sqrt{2}}$.
It is also possible to train a conditional diffusion models. We call the conditional diffusion architecture \cite{dhariwal2021diffusion} as CADM for short.
Correspondingly, UADM means the unconditional diffusion architecture.
UADM-G and CADM-G additionally use noise-aware classifier guidance to perform conditional generation, separately.

Our training hyperparameters of noise-aware classifier, including batch size, total number of iterations, and decay rate, are kept the same with Dhariwal \etal \cite{dhariwal2021diffusion} for fair comparison.
We adopt the fixed linear variance schedule $\beta_1,...,\beta_T$ \cite{nichol2021improved,ho2020denoising} for prior noising process Eq.\eqref{eq:rw_forward} and choose $T$ as $1000$.
In this paper, we set $\eta$ to 0.2 to keep a slight disturbance during training stage of classifier in all experiments. 
The selection details of $\gamma$ can be seen in supplementary materials.
All the experiments are conducted on 16 NVIDIA 3090s.
% Diffuison models in this paper are trained on Adam, with $\beta_1=0.9$ and $\beta_2=0.999$.
% we follow the architecture proposed in \cite{dhariwal2021diffusion} and train the guiding classifier with batch size 256. Hyperparameter $\eta$ is set to 0.2 for all result comparison and the number of training iterations is set to 500k.


% \vspace{-2pt}
\paragraph{\textbf{Evaluation Metrics.}}

We select FID (Fréchet Inception Distance) \cite{fid} as our default evaluation metric, which is the most widely used metric for generation evaluation.
FID \cite{fid} measures KL divergence of two Gaussian distributions, which is computed by the real reference samples and the generated samples, in the feature space of the Inception-V3. 
To capture more spatial relationships, sFID are prposed as a variant of FID, which is more sensitive to the consistent image distribution with high-level structures.

Besides, we apply several other metrics
% Inception Score (IS) \cite{noteoninceptionscore}, Improved Precision and Recall metrics \cite{precrecall} 
for more comprehensive evaluations.
Inception Score (IS) was proposed \cite{noteoninceptionscore},
to measure the mutual information between input sample and the predicted class.
Improved Precision and Recall metrics are proposed \cite{precrecall} for further evaluation of generative models.
% Two data manifolds are modeled by building explicit feature representations of the real and generated samples.
Precision is computed by estimating the proportion of generated samples that fall into real data manifold, measuring the sample fidelity.
By contraries, recall is computed by estimating the proportion of real samples which fall into generated data manifold, measuring the sample diversity.
% Usually, the more real and generated samples collected, the more accurate FID/sFID estimation is.
Following Dhariwal.et al \cite{dhariwal2021diffusion}, we randomly generated \textbf{50k} images to compute all metrics above based on \textbf{10k} real images when compared with previous methods.
For consistent comparisons, we use the evaluation metrics for all methods based on the same codebase as Dhariwal \etal \cite{dhariwal2021diffusion}.
% \vskip -0.2in
% Precision and IS are used to measure fidelity, and recall are used to measure diversity.
% sample fidelity is measured by computing the proportion of generated samples which fall into the real sample manifold
% Forming explicit non-parametric representations of the manifolds of real and generated data,
% \input{fig/compare_probability}


\subsection{Comparison with State-of-the-art Methods}

\input{table/sota256}
% \input{table/sota128-64}
% \input{table/sota256}
In this section, we show the comparison results of our proposed schemes with other SOTA methods.
based on UADM and CADM  architectures \cite{dhariwal2021diffusion}.
All results of other previous methods are cited from Dhariwal \etal \cite{dhariwal2021diffusion}.
% In Table.\ref{tab:sota}, we call this \textbf{CADM} for short.
% Correspondingly, we call unconditional architecture as \textbf{UADM}.
% Specifically, ADM-EDT means the DDPM are guided by the classifier trained with our proposed method EDT.
As shown in Table.\ref{tab:sota}, we achieve the best results in term of FID metric.
Compared with UADM-G in ImageNet 256$\times$256, our methods achieve relatively about 40\% improvement on FID metric (from 14.21 to 8.28, from 12.0 to 6.78) based on both DDPM and DDIM sampling iteration methods, with comparable or even better precision and recall.
When based on the CADM architecture, our proposed schemes still maintain a significant improvement margin on FID metric (from 5.44 to 4.67, from 4.59 to 4.09), and comparable precision and recall.

It is worth mentioning that our method based on UADM architecture outperformed BigGAN-deep in term of FID by 0.17 margin (6.78 vs 6.95), with no dependency on conditional architecture CADM, which has not been achieved in previous work \cite{dhariwal2021diffusion,ho2020denoising,nichol2021improved}.
\vspace{-6pt}
% Furthermore, our methods can be extended to low-resolution image data and get corresponding FID improvement (from 2.07 to 1.82, from 2.97 to 2.63), as shown in Table.\ref{tab:sota_lowr}.

% As a result, it can be verified that our proposed schemes can make a obvious generation quality improvement based on different architectures and iteration samplers (DDPM or DDIM)
.
% and achieve state-of-the-art results,
% For CADM-G,
% The results about ADM-G
% Furthermore, our methods barely add any computation cost and work well
% under different sampling methods, such as DDIM.

% We show the experiment results based on UADM in Table.\ref{tab:conditional}.
% When based on unconditional DDPM. our results are shown in Table.\ref{tab:unconditional}.
% In Table.\ref{tab:unconditional}, we show the results based on unconditional DDPM.
% From two tables, we can conclude that our proposed methods performed well based on different architectures and sampling methods, such as DDIM.
% It is worth mentioning that our method based on UADM architecture has already outperformed BigGAN-deep in term of FID, with no dependency on conditional architecture.

% When performing conditional diffusion generation guided by the classifier, 
% we also take concern of the the probability value to which the generated sample finally converges.
% In Figure.\ref{fig:gradnorm_and_p} (b), We plot the probability convergence curve of our methods and ADM-G, from which we can conclude that our proposed methods maintain
% more condition class information for generating samples.

% To further evaluate the performance of our proposed methods, 
% we show the quantitative results in Fig.\ref{fig:diversity}.
% Specifically, we sampled from the pretrained DDPM using ADM-G method and our proposed method respectively according to several class conditions.
% From the Fig.\ref{fig:diversity}, we can observe that the generated images sampled using our methods can preserve more texture details, in addition to accurate class condition information.

% with the improved training scheme EDT of the guiding classifier.
% Combined with our proposed sampling scheme EDS,
% generation results can be further improved.
% Furthermore, it can be observed that the performance improvement under conditional DDPM
% exceeds that under unconditional DDPM.
% The reason behind it is that the condition information involved in the training stage of 
% DDPM overcomes partly that brought by the classifier guidance.
% From the Table xxx,
% we summary that entropy-drive sampling method (EDS)
% is robust to many influencing factors of denoising sampling,
% including unconditional sampling methods, classifier scale, and diffusion steps.
% \input{table/ablation_eds}
% \vspace{-2pt}
\subsection{Ablation Study}
% \paragraph{\textbf{Effect of proposed schemes.}}
\subsubsection{Effect of proposed schemes.}
\label{exp:overall_ab}
% In this part, we perform several ablation experiments 
To further verify the contribution of each component of proposed schemes, we conduct ablation experiments on both UADM and CADM architectures, as shown in Table.\ref{tab:unconditional} and Table.\ref{tab:conditional}.
It can be concluded that EDS and ECT both improves the generation quality.
% proving the rationality of our motivation experimentally.
% Our motivation is proved experimentally
% Furthermore, ECT can assist EDS from training perspective, controlling the entropy scale within the reasonable numerical range.
Combining with two schemes, the generation results can be further improved, with more semantic details achieved from improved direction (ECT) and scale (EDS) aspects of guidance gradient.
% benefiting from the complementarity of EDS and ECT.
% With ECT scheme, the entropy-aware scaling factor in the later stage will be smoothed, avoiding the magnitude of numerial range.
% \vskip -0.2in
% \paragraph{\textbf{Effect of entropy-driven sampling.}}


\subsubsection{Effect of entropy-driven sampling.}
\label{exp:eds_ab}
\input{table/unconditional-ADM}
\input{table/conditional-ADM}
% The effect of EDS can mainly be attributed to its adaptation to various initial vanishing points and its reasonable recovering scale.
In this part, we design various intuitive scaling methods and compare them under optimal hyperparameters with EDS.
We select the scaling method with constant recovery factor for all time range \cite{dhariwal2021diffusion} as our baseline.

Intuitively, we can manually select vanishing time point through observing Fig.\ref{fig:vanishing_hist} and Fig.\ref{fig:coverge} i.e., 700, and finetune the constant rescaling factor to adjust the weak gradient for all generated samples, which we called Constant (range 0-700).
The constant scale can be further adjusted to time-aware form, such like $T-t$.
We call this method as Timestep-aware, which can dynamically adjust the scaling factor according to time step in sampling process.
In this way, the sample-aware vanishing characteristic is ignored and the scale cannot fit the various vanishing level.
% To verify that entropy-aware scale fit the sample-aware vanishing timestep, we design another approach based on entropy called Entropy-driven (Clip).

To verify that entropy-aware scaling could better fit the initial time steps of vanishing guidance, we design another approach which is based on norm of gradient map.
Specifically, we empirically select a norm bound $M$ for gradient.
When the norm of gradient map is smaller than the threshold vanishing norm bound $M$, we regard that the gradient guidance is weak and need to be rescaled.
Thus, $s$ in Eq.\ref{eq:condsample} is rewritten as followed:
\begin{equation} \label{eq:entropy_clip}
\begin{split}
s = \left\{
\begin{array}{rcl}
1, & & {\Vert \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t) \Vert_2 < M}\\
C,  & & \mathrm{Otherwise}\\
% F^*_R & & {S_M \leq 0 < S_R}\\
% F_R & & {S_R \leq 0}
\end{array} \right.
% \bg' &= \gamma * \frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t),
\end{split}
\end{equation}
The rescaling factor $C$ is a large constant.
Compared with methods above, it can be verified experimentally that EDS not only fits the sample-aware initial time steps of weak guidance, but also provides reasonable rescaling factor for recovery, as shown in Table.\ref{tab:ablation_EDS}.
% From Table.\ref{tab:ablation_EDS}, we can observe that little gain has achieved on above two intuitive scaling techniques.

% To verify that entropy-aware scale could fit the sample-aware vanishing timestep, we design another approach based on entropy called Entropy-driven (Clip).
% Specifically, we select a vanishing bound $M$ about entropy-aware scale, so that the EDS in Eq.\ref{eq:condsample} can be rewritten as followed:
% \begin{equation}\label{eq:entropy_clip}
% \begin{split}
% \bg' = \left\{
% \begin{array}{rcl}
% \gamma * \frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t), & & {\frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))} < M}\\
% M * \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t) & & \mathrm{Otherwise}\\
% % F^*_R & & {S_M \leq 0 < S_R}\\
% % F_R & & {S_R \leq 0}
% \end{array} \right.
% \end{split}
% \end{equation}
% In this way, the entropy-aware factor can only influence the vanishing time for each sample, while maintain the constant rescaling effect as Constant(0-700).
% From the Table.\ref{tab:ablation_EDS}, we can observe that Entropy-driven (Clip) can achieve obvious FID improvement, while it still performs not well as EDS.
% It can be verified that EDS not only fits the sample-aware vanishing time steps, but also provides reasonable rescaling factor for recovering weak guidance.

% \input{figure/augmented_finegrained_feature}
% \input{figure/finegrained_feature}
% \vspace{-4pt}
\input{table/ablation-eds}
\input{figure/gradient_map_vis}
\input{figure/compared_ddim25}
\subsection{Qualitative Results}
\subsubsection{Gradient Map Visualization.}
In this part, we collect several gradient maps $\bg$ derived from classifier in the previous sampling process and our EDS process, with an equal time interval.
From Fig.\ref{fig:grad_vis}, it can be observed that the classifier provides high-level semantic guidance at the beginning.
Gradually, the classifier will provide the condition-aware texture guidance.
Compared with EDS, which can maintain guidance of semantic details throughout the denoising process for refined generation results, sampling scheme based on the fixed scaling factor lost a lot of condition-aware details (first line) or introduce unnatural details (third line) at the later sampling stage.
% Compared with sampling scheme based on the fixed scaling factor, EDS can maintain guidance of semantic details throughout the denoising process for refined generation results, 
% while previous method lost a lot of condition-aware details (first line) or introduce unnatural details (third line) at the later sampling stage.

% For example, the first visualization class is trolleybus. The semantic details for that are geometric contour of vehicle. Obviously, our method can better maintain the contour.
% The second visualization class is jacamar.
% Our method can better preserve semantic details about bird's eyes, without unnatural details.

% \vspace{-2pt}
\subsubsection{Generation Results Visualization.}
In this part, we visualize various generated images conditioned on different classes.
Based on UADM architecture, we compared our final generated results with that of previous SOTA method \cite{dhariwal2021diffusion}.
Considering the stochastic noise involved in ddpm sampling process, we adopted DDIM, the deterministic generation process, to generate samples with shared initial noise.
% Previous method and ours shared with the same initial noise so that semantic details can be better compared
From Fig.(\ref{fig:comparation_results}), previous SOTA method can not generate condition-aware semantic details such like beaks of birds Fig.(\ref{fig:compare_1}) or petal texture Fig.(\ref{fig:compare_8}), while our method is able to generate more refined textures, with similar high-level structure.
% verifying the rationality of our motivation.
% We generated images based on original DDPM sampling method with 250 steps for UADM-G and our methods. From Fig.\ref{fig:diversity} (b), it can be observed that our generation quality is better than UADM-G.
% We mainly focus
% Further ablation experiments are conducted on CASIAB to demonstrate the positive impact of each component in our method. 
% It should be noted that, our baseline does not contain any of the proposed modules in this paper.
% \textbf{Effectiveness of entropy-constrain training scheme.}
% % plot figure to show the performance FID
% For efficiency, we perform experiments based on Tiny ImageNet.
% For modeling noisy label, the intuitive approach is to
% perturb the original label $y$ by the Gaussian transition kernel
% with hyper-parameter $\sigma$.
% We set $\sigma$ to $1$ to control the variance range.
% We generate 5k samples separately and evaluate them based on FID.

% \textbf{Effectiveness of entropy-driven sampling scheme.}
% There are many approaches to design dynamic scaling factors.
% Intuitively, the linear scaling scheme can be considered,
% which designed the scaling factor as a linear function about timestep $t$,
% so the same as the cosine scaling scheme.
% To be specific, we design the linear function as $ T - t$ to be roughly consistent with the change law of entropy 

% From the perspective of prior data statistics, we consider the scaling scheme based on 
% the gradient variation law estimated from real data and its diffusion prior.
% More details can be seen in supplementary materials.

% The comparison results are shown in Table.\ref{tab:ablation_EDS},
% which is evaluated based on DDIM sampling method with $25$ timesteps and unconditional DDPM architecture.
% \subsection{Visualization}

% \input{figure/compared_ddpm250}
% \vspace{-0.1cm}
\section{Conclusion}
In this paper, we proposed an entropy-aware scaling technology for the guiding classifier in sampling process.
% The key insight is to alleviate the early vanishing of gradient guidance from classifier.
From the perspective of training, we propose an entropy-aware optimization loss to constrain the predicted distribution, alleviating the overconfident prediction for noisy sample in the sampling process.
% constrain the sparsity of predicted distribution by optimizing its entropy.
% From the perspective of sampling, we utilize the entropy to rescale the guiding gradient to make sure its robustness.
Experiments demonstrate that our proposed methods can recover more textures in generated samples,
achieving state-of-the-art generation results.
% outperform existing others and achieve state-of-the-art results on ImageNet benchmark in term of FID metric.
% the effectiveness of our proposed methods 



==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/algorithm/entropy-DDIM-sampling.tex <==
\algrenewcommand\algorithmicindent{0.5em}%
\begin{algorithm}[t]
    \caption{\small{Entropy-driven sampling scheme (DDIM), given a pretrained diffusion model $\epsilon_{\theta}(\bx_t)$, classifier $p_{\phi}(\tilde \by_t|\bx_t)$, and desired class condition $y$.}}
    \label{alg:entropy_driven_ddim}
    \begin{algorithmic}[1]
        \State $\bx_T \sim \mathcal{N}(\bzero, \bI)$
        \For{$t=T, \dotsc, 1$}
            % \State $\bz \sim \mathcal{N}(\bzero, \bI)$ if $t > 1$, else $\bz = \bzero$
            \State $\hbepsilon = \bepsilon_{\theta}(\bx_t) - \gamma * \frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t),$
            \State $\bx_{t-1} = \sqrt{\bar \alpha_{t-1}}(\frac{\bx_t - \sqrt{1- \bar \alpha_t}\hbepsilon}{\sqrt{\bar \alpha_t}}) 
            + \sqrt{1-\bar \alpha_{t-1}}\hbepsilon$
            % \State $\bx_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left( \bx_t - \frac{1-\alpha_t}{\sqrt{1-\bar\alpha_t}} \hbepsilon_\theta(\bx_t) \right) + \sigma^2_t \bg + \sigma_t \bz$
        \EndFor
        \State \textbf{return} $\bx_0$
    \end{algorithmic}
\end{algorithm}


==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/algorithm/entropy-DDPM-sampling.tex <==
\algrenewcommand\algorithmicindent{0.5em}%
\begin{algorithm}[t]
    \caption{ \small{Entropy-driven sampling scheme (DDPM), given a pretrained diffusion model $\epsilon_{\theta}(\bx_t)$, classifier $p_{\phi}(\hat \by_t|\bx_t)$, and desired class condition $\by$.}}
    \label{alg:entropy_driven_ddpm}
    \begin{algorithmic}[1]
        \State $\bx_T \sim \mathcal{N}(\bzero, \bI)$
        \For{$t=T, \dotsc, 1$}
            \State $\bz \sim \mathcal{N}(\bzero, \bI)$ if $t > 1$, else $\bz = \bzero$
            \State $\bg = \gamma * \frac{\mathcal{H}(\mathcal{U}(\hat \by))}{\mathcal{H}(p_{\phi}(\hat \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t),$
            \State $\bx_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left( \bx_t - \frac{1-\alpha_t}{\sqrt{1-\bar\alpha_t}} \bepsilon_\theta(\bx_t) \right) + \sigma^2_t \bg + \sigma_t \bz$
        \EndFor
        \State \textbf{return} $\bx_0$
        % \RETURN $\phi$
    \end{algorithmic}
\end{algorithm}


==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/algorithm/entropy-sampling.tex <==
% \algrenewcommand\algorithmicindent{0.5em}%


% \columnseprule=1pt         % 实现插入分隔线
%  \begin{multicols}{2} 
  
\begin{algorithm}[t]
    \caption{ \small{Entropy-driven sampling scheme (DDPM/DDIM)}}
    \label{alg:entropy_driven_ddpm}
        
    \begin{algorithmic}[1]
        \Require a pretrained diffusion model $\epsilon_{\theta}(\bx_t)$, classifier $p_{\phi}(\hat \by|\bx_t)$, and desired class condition $\by$
        \State $\bx_T \sim \mathcal{N}(\bzero, \bI)$
        \For{$t = T, \dotsc, 1$}
            \State $s \gets \gamma * \frac{\mathcal{H}(\mathcal{U}(\hat \by))}{\mathcal{H}(p_{\phi}(\hat \by|\bx_t))}$ if EDS, else $s \gets \gamma$
    
            \If{use DDPM}
                \State $\bz \sim \mathcal{N}(\bzero, \bI)$ if $t > 1$, else $\bz \gets \bzero$
                
                \State $\bg \gets  s \cdot \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t),$
                
                \State $\bx_{t-1} \gets \frac{1}{\sqrt{\alpha_t}}\left( \bx_t - \frac{1-\alpha_t}{\sqrt{1-\bar\alpha_t}} \bepsilon_\theta(\bx_t) \right) + \sigma^2_t \bg + \sigma_t \bz$
            \ElsIf{use DDIM}
                \State $\hbepsilon \gets \bepsilon_{\theta}(\bx_t) -  s \cdot \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t),$
                
                \State $\bx_{t-1} \gets \sqrt{\bar \alpha_{t-1}}(\frac{\bx_t - \sqrt{1- \bar \alpha_t}\hbepsilon}{\sqrt{\bar \alpha_t}}) 
                + \sqrt{1-\bar \alpha_{t-1}}\hbepsilon$
            \EndIf
        \EndFor
        \State \textbf{return} $\bx_0$
        
        % \RETURN $\phi$
    \end{algorithmic}
    
  
\end{algorithm}

% \begin{algorithm}[]
%     \caption{\small{Entropy-constraint training scheme.
%     }}
%     \label{alg:entropy_constraint_train}
    
%     \begin{algorithmic}[1]
%         \Require training set $\mathbb{D}$, a neural classifier $\phi$, training set $\mathbb{D}$, total time steps $T$
%         \Repeat
%             \State $(\bx_0,\by) \gets \text{sample from } \mathbb{D}$
%             \State $t \sim \mathcal{U}(\{1, \dotsc ,T\})$
%             \State $\bx_t \sim q(\bx_t|\bx_0)$ (Eq.\ref{eq:sample_diffusion})
%             \State $L_{CE} \gets \by \log p_{\phi}(\tilde \by|\bx_t)$
            
%             \If{use ECT}
%                 \State $L_{ECT} \gets - \mathcal{H}(p_{\phi}(\tilde \by|\bx_t)) $
%                 \State Take gradient descent step on $\nabla_{\phi} ( L_{CE} + \eta L_{ECT})$
%             \Else
%                 \State Take gradient descent step on $\nabla_{\phi}  L_{CE}$
%             \EndIf
%         \Until{converged}
%         % \RETURN $\phi$
%     \end{algorithmic}
% \end{algorithm}

% \end{multicols}



==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/algorithm/entropy-training.tex <==
% \algrenewcommand\algorithmicindent{0.5em}%
\begin{algorithm}[!t]
    \caption{\small{Entropy-constraint training scheme.
    }}
    \label{alg:entropy_constraint_train}
    
    \begin{algorithmic}[1]
        \Require training set $\mathbb{D}$, a neural classifier $\phi$, training set $\mathbb{D}$, total time steps $T$
        \Repeat
            \State $(\bx_0,\by) \gets \text{sample from } \mathbb{D}$
            \State $t \sim \mathcal{U}(\{1, \dotsc ,T\})$
            \State $\bx_t \sim q(\bx_t|\bx_0)$ (Eq.\ref{eq:sample_diffusion})
            \State $L_{CE} \gets \by \log p_{\phi}(\tilde \by|\bx_t)$
            
            \If{use ECT}
                \State $L_{ECT} \gets - \mathcal{H}(p_{\phi}(\tilde \by|\bx_t)) $
                \State Take gradient descent step on $\nabla_{\phi} ( L_{CE} + \eta L_{ECT})$
            \Else
                \State Take gradient descent step on $\nabla_{\phi}  L_{CE}$
            \EndIf
        \Until{converged}
        % \RETURN $\phi$
    \end{algorithmic}
\end{algorithm}


==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/algorithm/test.tex <==
\begin{algorithm}[t]
 \caption{\textbf{\label{alg:GraphBuild}}Inference graph building}
 {

 \textbf{\small{{Input:}}}{\small{
 CNN $CN$, a set $\Omega$ of images predicted by $CN$ to class $m$, network model ${\{ \Theta^l, \hat{P}(h^l=k), \hat{P}(h^l=k|h^{l'}=k')  \}}_{l=1, k=1,k'=1}^{L,K^l,K^{l'}}$,
$Z$ - number of allowed nodes per layer.
 \textbf{\small{Output:}}{
 \small{An inference graph $G=(N,E)$, where $N$ and $E$ hold clusters (nodes) and their weighted connections (edges) in the graph, respectively
 %with 

 %$N=C^L_m \cup  {\{ C^l_{z^l_i}  \}}_{l=1, i=1}^{L-1,Z}$ and 
 %$E={\{e^l_{i,j}\}}_{l=1,i=1,j=1}^{L-1,Z,Z}$ 
  }} 

 \textbf{\small{Initialization:}} 
 Push $\Omega$ through the network model to get ${\{ Q^l_{t,s}(\Omega)\}}_{l=1}^{L-1}$ (Eq.~\ref{eq:Q_t,s(omega)}) and clusters ${\{C^l_i\}}_{l=1,i=1}^{L,K^l}$.
~{\small
Set $S=m$, $N=C^L_m$, and $E=\emptyset$ %//m is the index of the output cluster to explain }
%\quad $N=S$ } 
 
 {\small For $l=L-1,\dots, 1$ }
 
% {\small{{$~~~$ Set $l= l'+1$  }}}

 {\small{{$~~~$ For $t=1,\dots,K^{l}$}}}, {\small{compute $S^{l}(\Omega,S,t)$ (Eq.~\ref{eq:OmageScore})}}

 {\small{{$~~~$ Choose $(z^{l}_1,\dots,z^{l}_Z)$ to be the $Z$ clusters indices with the largest scores $S^{l}(\Omega,S,t)$  }}}

 {\small{$~~~$ Set $S= (z^{l}_1,\dots,z^{l}_Z)$ and  $e^{l}_{i,j} = S^{l}(\Omega,z^{l+1}_i,z^{l}_j)$, $\forall i,j=1,\dots Z$ } }
 
 {\small{$~~~$ Set $N=N\cup{\{C^l_{z^l_i}\}}_{i=1}^Z$ and $E=E\cup{\{e^l_{i,j}\}}_{i=1,j=1}^{Z,Z}$ }}// nodes and edges update
%\quad $N= N \cup S$}}

% {\small{{$~~~$ Set $N= N \cup S$  }}}
  }}} }
 \end{algorithm}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/figure/compared_ddim25.tex <==
\begin{figure}[!t]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class1.pdf}
         \caption{Class 1:goldfish}
         \label{fig:compare_0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class13.pdf}
         \caption{Class 13:junco}
         \label{fig:compare_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class22.pdf}
         \caption{Class 22:eagle}
         \label{fig:compare_2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class5.pdf}
         \caption{Class 5:numbfish}
         \label{fig:compare_3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class923.pdf}
        %  \caption{$y=3sinx$}
         \caption{Class 923:plate}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class874.pdf}
         \caption{Class 874:trolleybus}
         \label{fig:compare_5}
     \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class984.pdf}
         \caption{Class 984:rapeseed}
         \label{fig:compare_6}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class970.pdf}
         \caption{Class 970:alp}
         \label{fig:compare_7}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/class985.pdf}
         \caption{Class 985:daisy}
         \label{fig:compare_8}
     \end{subfigure}
    \caption{
    % Comparison of generated samples (256$\times$256) from fixed scaling sampling \cite{dhariwal2021diffusion} and ours (ECT+EDS) based on UADM. The iteration sampler is based on DDIM and the iteration steps are set to 25. For all image blocks, the first line is generated from previous method while the second line from ours. 
    Sample quality comparison of UADM-G \cite{dhariwal2021diffusion} (the first line of each image box) and our UADM-G + ECT + EDS (the second line of each image box) on ImageNet1000 256$\times$256 using DDIM 25 iterations. 
    }
    \label{fig:comparation_results}
    \vskip -0.2in
\end{figure}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/figure/compared_ddpm250.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/compared_baseline.pdf}
         \caption{$y=x$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/compared_ECT+EDS.pdf}
         \caption{$y=3sinx$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{0.3\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{graph3}
    %      \caption{$y=5/x$}
    %      \label{fig:five over x}
    %  \end{subfigure}
        \caption{Three simple graphs}
        \label{fig:three graphs}
\end{figure}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/figure/finegrained_feature.tex <==
\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=1.0\textwidth]{figure/finegrained_feature.jpg}
    \caption{vanishing fine-grained feature in normal inference}\label{fig:finegrained_feature}
    \end{center}
    \vskip -0.2in
\end{figure}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/figure/first_img.tex <==
% \begin{figure}[!t]
%     \begin{center}
%         \subfigure{\includegraphics[width=0.5\textwidth]{fig/grad_norm_and_probability_baseline.pdf}} 
%     	\subfigure{\includegraphics[width=0.5\textwidth]{fig/grad_norm_and_probability_ECT+EDS.pdf}}
%         \includegraphics[width=3.3in,height=2.5in]{fig/grad_norm_and_probability_baseline.pdf}
%     \end{center}
%     \caption{The effect of changing temperature for an ImageNet 128$\times$128 model.} 
%     \label{fig:gradnorm_and_p}
% \end{figure}

\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=0.87\textwidth]{figure/first_img_fig.pdf}
    % \begin{subfigure}[(a) previous method]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{fig/grad_norm_and_probability_baseline4.pdf}
    % \end{subfigure}
    % % \hspace{0.025\textwidth}
    % \begin{subfigure}[(b) ours]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{fig/grad_norm_and_probability_ECT+EDS4.pdf}
    % \end{subfigure}
    \caption{
    % The curves of predicted probability and gradient norm for baseline and our method.
    % We make statistics of the gradient norms based on multiple samples. For better display, we show one of the statistical curves and its corresponding denoising samples.
    The visualization of denoising sampling process. The classifier gradient, a kind of class information in conditional generation, quickly converge to 0 in the previous method. It will lead to the collapse from conditional generation to unconditional generation, while our method recovers the gradient guidance and succeed to generate fine-grained features in the subsequent iterations.
    % When the predicted probability approaches to 1.0, the guiding gradient of previous method decays to nearly 0, while our methods still maintain it, recovering more conditional semantic details.
    }\label{fig:coverge}
   
    \end{center}
    \vskip -0.2in
\end{figure}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/figure/gradient_map_vis.tex <==
\begin{figure}[!t]
    \vspace{-3pt}
    \begin{center}
    \includegraphics[width=1.0\textwidth]{figure/gradient_map_vis_fig.pdf}
    \caption{Gradient map comparison of UADM-G \cite{dhariwal2021diffusion} (the first line of each image box) and our UADM-G + EDS (the second line of each image box) on ImageNet1000 256$\times$256 using DDIM 25 iterations. For better visualization, we pick 8 maps at the same interval from 25 consecutive maps and magnify all pixels of a image by a factor of 50.
    }\label{fig:grad_vis}
    \end{center}
    \vspace{-8mm}
\end{figure}




==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/figure/pipeline.tex <==
% \begin{figure}[!t]
%     \begin{center}
%         \subfigure{\includegraphics[width=0.5\textwidth]{fig/grad_norm_and_probability_baseline.pdf}} 
%     	\subfigure{\includegraphics[width=0.5\textwidth]{fig/grad_norm_and_probability_ECT+EDS.pdf}}
%         \includegraphics[width=3.3in,height=2.5in]{fig/grad_norm_and_probability_baseline.pdf}
%     \end{center}
%     \caption{The effect of changing temperature for an ImageNet 128$\times$128 model.} 
%     \label{fig:gradnorm_and_p}
% \end{figure}

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1.\textwidth]{figure/pipeline_fig.pdf}
    % \begin{subfigure}[(a) previous method]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{fig/grad_norm_and_probability_baseline4.pdf}
    % \end{subfigure}
    % % \hspace{0.025\textwidth}
    % \begin{subfigure}[(b) ours]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{fig/grad_norm_and_probability_ECT+EDS4.pdf}
    % \end{subfigure}
    \caption{Pipeline for Entropy-driven Sampling process. Sampler represents a class of iteration method (DDPM or DDIM), which is non-parametric. All models are pretrained without gradient updating in the sampling process.}\label{fig:pipeline}
    \end{center}
    \vskip -0.2in
\end{figure}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/figure/vanishing_point_hist.tex <==
\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=1.0\textwidth]{figure/vanishing_point_hist_fig.jpg}
    \caption{The various gradient vanishing points for different samples. We randomly generate 5000 samples and define the time point, in which the gradient norm is smaller than 0.15, as the gradient vanishing point. Premature vanishing of gradients occurs in almost every sample.}\label{fig:vanishing_hist}
    \end{center}
    \vskip -0.3in
\end{figure}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/table/ablation-eds.tex <==
\begin{table}[t]
    \setlength\tabcolsep{3.5mm}
    \caption{Sample quality comparison with several intuitive sampling schemes. All results are evaluated under 5,000 generated samples for more efficient comparisons.}\label{tab:ablation_EDS}
    \begin{center}
    % \begin{small}
    % \begin{subtable}[t]{.5\linewidth}
    \begin{tabular}[t]{lcccc}
    \toprule
    Method            & FID          & IS       & Precision      & Recall \\
    % \multicolumn{5}{l}{\bf{ImageNet} 256$\times$256} \\
    \toprule
    Baseline  & 20.17        & 84.53          & 0.71          & 0.59       \\
    % Linear                  & 10.94         & 6.02          & 0.69          & 0.63       \\
    % Tanh      & 5.44	         & 5.32          & 0.81	         & 0.49       \\
    Constant (range 0-700)      & 19.84	       & 88.42          & 0.70	         & 0.61       \\
    Timestep-aware & 19.42    & 87.42          & 0.70	         & 0.63       \\
    % Variance-aware      & 5.44	         & 5.32          & 0.81	         & 0.49       \\
    % Data-driven         & 4.59     & 5.25     & 0.82          & 0.52       \\
    % Probability-driven               & 4.59     & 5.25     & 0.82          & 0.52       \\
    % Partly constant Scale               & 4.59     & 5.25     & 0.82          & 0.52       \\
    % Entropy-driven (Clip)               & 17.24     & 118.85     & \bf 0.73          & 0.64       \\
    Gradient Norm               & 19.08     & 93.14     & 0.71          & 0.63       \\
    Entropy-driven  & \bf 16.56    & \bf 133.26     & \bf 0.73          & \bf 0.66       \\
    \toprule
    \end{tabular}
    % \end{subtable}
    % \end{small}
    \end{center}
    \vspace{-1pt}
\end{table}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/table/conditional-ADM.tex <==
\begin{table}[!t]
    % \vspace{-2mm}
    \caption{Effect of our proposed methods based on CADM-G under DDIM 25 steps and DDPM 250 steps on ImageNet1000 256$\times$256.}
    \label{tab:conditional}
    \begin{center}
    % \begin{small}
    \setlength{\tabcolsep}{1.8mm}{
    \begin{tabular}{cccccccc}
    \toprule
    DDIM & ECT & EDS & FID $\downarrow$   & sFID $\downarrow$ & IS $\uparrow$  & Precision $\uparrow$ & Recall $\uparrow$  \\
    \midrule
        & &      & 4.59 & 5.25  & 186.7  & 0.82      & 0.52 \\
         & \cmark &   & 4.62 & 5.16 & 182.48  & 0.81      & \bf 0.53 \\
         & & \cmark  & \bf 4.01 & 5.15 & 217.25  & 0.82      & 0.52 \\
         & \cmark & \cmark & 4.09 & \bf 5.07 & \bf 221.57  & \bf 0.83      & 0.50 \\
    \hline
    
        \cmark &  &     & 5.46 & 5.32  & 194.48  & 0.81      & 0.48 \\
         \cmark &  \cmark &   & 5.34 & 5.3 & 196.8  & 0.81      & 0.49 \\
          \cmark &  & \cmark   & 4.82 & \bf 5.04 & 218.97  & 0.80      & \bf 0.50 \\
         \cmark & \cmark & \cmark &\bf 4.67 & 5.12 & \bf 235.24  & \bf 0.82      & 0.48 \\
    \bottomrule
    \end{tabular}
    }
    % \end{small}
    \end{center}
    % \vskip -0.33in
    \vspace{-4mm}
\end{table}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/table/sota128-64.tex <==
\begin{table}[t]
    \setlength\tabcolsep{2.5mm}
    \caption{\textbf{Comparison results with state-of-the-art generative models based on ImageNet 128$\times$128, 64$\times$64.} Annotation '(25 )' after the method means its sampling process is based on DDIM with 25 steps. Otherwise, it means the normal sampling method in DDPM, with 250 steps.}
    \label{tab:sota_lowr}
    \begin{center}
    % \small
    % \begin{small}
    
    % \begin{subtable}[t]
    \begin{tabular}[t]{lcccc}
    \toprule
    Method            & FID $\downarrow$         & sFID  $\downarrow$     & Prec  $\uparrow$    & Rec $\uparrow$ \\
    \\
    \multicolumn{5}{l}{\bf{ImageNet} 64$\times$64} \\
    \toprule
    BigGAN-deep \cite{bigbigan}    & 4.06         & 3.96      & \bf{0.79} & 0.48  \\
    IDDPM    \cite{improved} & 2.92         & \bf{3.79} & 0.74      & 0.62 \\
    % CADM-G             & 2.61         & \bf{3.77} & 0.73      & 0.63  \\
    \toprule
    CADM-G  \cite{dhariwal2021diffusion} & 2.07   & 4.29      & 0.74      & \bf{0.63}  \\
    \bf{CADM-G+EDS+ECT}                & \bf{1.88}	 & 4.51     & 0.76          & 0.61          \\
    % \toprule
    % \begin{subtable}[t]{.5\linewidth}
    % \begin{tabular}[t]{lcccc}
    % \toprule
    % Model            & FID          & sFID       & Prec & Rec \\
    \\
    \multicolumn{5}{l}{\bf{ImageNet} 128$\times$128} \\
    
    \toprule
    BigGAN-deep  \cite{bigbigan}           & 6.02          & 7.18          & \bf{0.86}     & 0.35          \\
    LOGAN   \cite{logan} & 3.36          &               &               &               \\
    CADM    \cite{dhariwal2021diffusion}                     & 5.91          & 5.09     & 0.70          & \bf{0.65}     \\
    \toprule
    CADM-G (25)   \cite{dhariwal2021diffusion}   & 6.58          & 7.52          & 0.77          & 0.50          \\
    \bf{CADM-G+EDS+ECT (25)}                & 6.22	 & 7.10     & 0.78          & 0.49          \\
    % \toprule
    CADM-G    \cite{dhariwal2021diffusion}            & 2.97	 & \bf{5.09}     & 0.78          & 0.59          \\
    \bf{CADM-G+EDS+ECT}                & \bf{2.68}	 & 5.10     & 0.80          & 0.56        \\
    \toprule
    
    \end{tabular}
    % \end{subtable}
    % \begin{subtable}[t]{.5\linewidth}
    % \begin{tabular}[t]{lcccc}
    
    % \toprule
    % Method            & FID $\downarrow$         & sFID  $\downarrow$     & Prec  $\uparrow$    & Rec $\uparrow$ \\
    % \\
    
    % \multicolumn{5}{l}{\bf{ImageNet} 256$\times$256} \\
    % \toprule
    % DCTransformer            & 36.51         & 8.24          & 0.36          & \bf{0.67}  \\

    % VQ-VAE-2 & 31.11 & 17.38 & 0.36 & 0.57 \\
    % IDDPM & 12.26 & 5.42 & 0.70 & 0.62 \\
    % SR3 & 11.30 & & & \\
    % BigGAN-deep             & 6.95          & 7.36          & \bf{0.87}     & 0.28       \\
    % UADM-G  (25)                & 14.21         & 8.53          & 0.7          & 0.46       \\
    % UADM-G                & 12         & 10.4          & 0.76          & 0.44       \\
    % CADM                  & 10.94         & 6.02          & 0.69          & 0.63       \\
    % CADM-G (25)    & 5.44	         & 5.32          & 0.81	         & 0.49       \\
    % CADM-G              & 4.59     & 5.25     & 0.82          & 0.52       \\
    % \toprule
    % \bf{UADM-G + ECT + EDS} (25)                & 8.28      & 6.37     & 0.76          & 0.44     \\
    % \bf{UADM-G + ECT + EDS}            & 6.78     & 6.56     & 0.81          & 0.45     \\
    % \bf{CADM-G + ECT + EDS} (25)                & 4.67      & 5.12     & 0.82          & 0.47     \\
    % \bf{CADM-G + ECT + EDS}            & \bf{4.09}     & \bf{5.07}     & 0.83          & 0.50     \\
    % \toprule
    % \end{tabular}
    % \end{subtable}
    
    % \end{small}
    \end{center}
    
    
    
    \vskip -0.2in
\end{table}



% \begin{table*}[th]
%     \setlength\tabcolsep{6pt}
%     \begin{center}
%     % \begin{small}
    
%     % \begin{subtable}[t]{.5\linewidth}
%     % \setlength{\tabcolsep}{5mm}{
%     \begin{tabular}[t]{lcccc}
%     \toprule
%     Method            & FID $\downarrow$         & sFID  $\downarrow$     & Precision  $\uparrow$    & Recall $\uparrow$ \\
    
%     % \multicolumn{5}{l}{\bf{ImageNet} 256$\times$256} \\
%     \toprule
%     DCTransformer${}^\dagger$ \cite{dctransformer}            & 36.51         & 8.24          & 0.36          & \bf{0.67}  \\
%     % IDDPM \shortcite{improved} & 31.50 & 20.27 & 0.65 & 0.60 \\
    
%     % VQ-VAE-2 vqvae2
%     % IDD improved
%     % sr3 sr3
%     % Biggan biggan
%     % ADM dhariwal
%     VQ-VAE-2${}^\dagger{}^\ddag$ \cite{vqvae2} & 31.11 & 17.38 & 0.36 & 0.57 \\
%     IDDPM${}^\ddag$ \cite{improved} & 12.26 & 5.42 & 0.70 & 0.62 \\
%     SR3${}^\dagger{}^\ddag$ \cite{sr3} & 11.30 & & & \\
%     BigGAN-deep \cite{biggan}             & 6.95          & 7.36          & \bf{0.87}     & 0.28       \\
%     ADM      \cite{dhariwal2021diffusion}            & 10.94         & 6.02          & 0.69          & 0.63       \\
%     ADM-G (25 steps)  \cite{dhariwal2021diffusion}  & 5.44	         & 5.32          & 0.81	         & 0.49       \\
%     ADM-G    \cite{dhariwal2021diffusion}          & 4.59     & 5.25     & 0.82          & 0.52       \\
%     \toprule
%     \bf{ADM-EDT} (25 steps)                     & 5.34         & 5.3         & 0.81          & 0.49      \\
%     \bf{ADM-EDT}      & 4.62	         & 5.16         & 0.81	         & 0.53       \\
%     \bf{ADM-EDT + EDS} (25 steps)                & 4.81      & 5.22     & 0.83          & 0.45     \\
%     \bf{ADM-EDT + EDS}             & \bf{4.09}     & \bf{5.07}     & 0.83          & 0.50     \\
%     \toprule
%     \end{tabular}
%     % \end{subtable}
    
%     % \end{small}
%     \end{center}
%     \caption{Sample quality comparison with state-of-the-art generative models for each task.}
    
%     \label{tab:sota}
% \end{table*}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/table/sota256.tex <==
\begin{table}[t]
    \setlength\tabcolsep{2.5mm}
    \caption{Comparison results with state-of-the-art generative models on ImageNet1000 256$\times$256. Annotation '(25)' means the DDIM \cite{ddim} sampling method with 25 steps. Otherwise, it means DDPM sampling method with 250 steps.
    }\label{tab:sota}
    \begin{center}
    % \small
    % \begin{small}
    
    % \begin{subtable}[t]{.5\linewidth}
    % \begin{tabular}[t]{lcccc}
    % \toprule
    % Method            & FID $\downarrow$         & sFID  $\downarrow$     & Prec  $\uparrow$    & Rec $\uparrow$ \\
    % \\
    % \multicolumn{5}{l}{\bf{ImageNet} 64$\times$64} \\
    % \toprule
    % BigGAN-deep     & 4.06         & 3.96      & \bf{0.79} & 0.48  \\
    % IDDPM    & 2.92         & 3.79 & 0.74      & 0.62 \\
    % CADM-G             & 2.61         & \bf{3.77} & 0.73      & 0.63  \\
    % CADM-G (dropout)   & 2.07   & 4.29      & 0.74      & \bf{0.63}  \\
    % \toprule
    % \bf{CADM-G (dropout)+ EDS}                & \bf{1.82}	 & 4.33     & 0.76          & 0.61          \\
    % % \toprule
    % % \begin{subtable}[t]{.5\linewidth}
    % % \begin{tabular}[t]{lcccc}
    % % \toprule
    % % Model            & FID          & sFID       & Prec & Rec \\
    % \\
    % \multicolumn{5}{l}{\bf{ImageNet} 128$\times$128} \\
    
    % \toprule
    % BigGAN-deep             & 6.02          & 7.18          & \bf{0.86}     & 0.35          \\
    % LOGAN${}^\dagger$   & 3.36          &               &               &               \\
    % CADM                     & 5.91          & 5.09     & 0.70          & \bf{0.65}     \\
    % CADM-G (25)      & 6.58          & 7.52          & 0.77          & 0.50          \\
    % CADM-G                & 2.97	 & 5.09     & 0.78          & 0.59          \\
    
    % \toprule
    % \bf{CADM-G + EDS (25)}                & 6.18	 & 7.10     & 0.78          & 0.49          \\
    % \bf{CADM-G + EDS}                & \bf{2.63}	 & \bf{4.94}     & 0.79          & 0.58          \\
    % % \toprule
    
    % \end{tabular}
    % \end{subtable}
    % \begin{subtable}[t]{.5\linewidth}
    \begin{tabular}[t]{lccccc}
    
    \toprule
    Method            & FID $\downarrow$         & sFID  $\downarrow$ & IS $\uparrow$     & Prec  $\uparrow$    & Rec $\uparrow$ \\
    % \\
    
    % \multicolumn{6}{l}{\bf{ImageNet} 256$\times$256} \\
    \toprule
    DCTransformer \cite{dctransformer} & 36.51 & 8.24 & - & 0.36 & \bf{0.67}  \\
    VQ-VAE-2 \cite{vqvae2}    & 31.11 & 17.38 & - & 0.36 & 0.57 \\
    IDDPM \cite{nichol2021improved}   & 12.26 & 5.42 & - & 0.70 & 0.62 \\
    SR3  \cite{sr3}  & 11.30 & - & - & - & -\\
    BigGAN-deep \cite{biggan}  & 6.95 & 7.36 & - & \bf{0.87} & 0.28\\
    \toprule
    UADM-G  \cite{dhariwal2021diffusion}(25)  & 14.21 & 8.53 & 83 & 0.7 & 0.46 \\
    \bf{UADM-G+ECT+EDS} (25) & 8.28 & 6.37 & 163.17 & 0.76 & 0.44 \\
    UADM-G  \cite{dhariwal2021diffusion}   & 12 & 10.4 & 95.41 & 0.76 & 0.44 \\
    \bf{UADM-G+ECT+EDS} & 6.78 & 6.56 & 168.78 & 0.81 & 0.45 \\
    \toprule
    CADM   \cite{dhariwal2021diffusion}     & 10.94 & 6.02 & 100.98 & 0.69 & 0.63 \\
    CADM-G (25)  \cite{dhariwal2021diffusion}  & 5.44 & 5.32 & 194.48 & 0.81 & 0.49 \\
    \bf{CADM-G+ECT+EDS} (25) & 4.67 & 5.12 & \textbf{235.24} & 0.82 & 0.47     \\
    CADM-G \cite{dhariwal2021diffusion} & 4.59 & 5.25 & 186.70 & 0.82 & 0.52 \\
    \bf{CADM-G+ECT+EDS} & \bf{4.09} & \bf{5.07} & 221.57 & 0.83 & 0.50 \\
    \toprule
    \end{tabular}
    % \end{subtable}
    
    % \end{small}
    \end{center}
    \vspace{-2pt}
\end{table}



% \begin{table*}[th]
%     \setlength\tabcolsep{6pt}
%     \begin{center}
%     % \begin{small}
    
%     % \begin{subtable}[t]{.5\linewidth}
%     % \setlength{\tabcolsep}{5mm}{
%     \begin{tabular}[t]{lcccc}
%     \toprule
%     Method            & FID $\downarrow$         & sFID  $\downarrow$     & Precision  $\uparrow$    & Recall $\uparrow$ \\
    
%     % \multicolumn{5}{l}{\bf{ImageNet} 256$\times$256} \\
%     \toprule
%     DCTransformer${}^\dagger$ \cite{dctransformer}            & 36.51         & 8.24          & 0.36          & \bf{0.67}  \\
%     % IDDPM \shortcite{improved} & 31.50 & 20.27 & 0.65 & 0.60 \\
    
%     % VQ-VAE-2 vqvae2
%     % IDD improved
%     % sr3 sr3
%     % Biggan biggan
%     % ADM dhariwal
%     VQ-VAE-2${}^\dagger{}^\ddag$ \cite{vqvae2} & 31.11 & 17.38 & 0.36 & 0.57 \\
%     IDDPM${}^\ddag$ \cite{improved} & 12.26 & 5.42 & 0.70 & 0.62 \\
%     SR3${}^\dagger{}^\ddag$ \cite{sr3} & 11.30 & & & \\
%     BigGAN-deep \cite{biggan}             & 6.95          & 7.36          & \bf{0.87}     & 0.28       \\
%     ADM      \cite{dhariwal2021diffusion}            & 10.94         & 6.02          & 0.69          & 0.63       \\
%     ADM-G (25 steps)  \cite{dhariwal2021diffusion}  & 5.44	         & 5.32          & 0.81	         & 0.49       \\
%     ADM-G    \cite{dhariwal2021diffusion}          & 4.59     & 5.25     & 0.82          & 0.52       \\
%     \toprule
%     \bf{ADM-EDT} (25 steps)                     & 5.34         & 5.3         & 0.81          & 0.49      \\
%     \bf{ADM-EDT}      & 4.62	         & 5.16         & 0.81	         & 0.53       \\
%     \bf{ADM-EDT + EDS} (25 steps)                & 4.81      & 5.22     & 0.83          & 0.45     \\
%     \bf{ADM-EDT + EDS}             & \bf{4.09}     & \bf{5.07}     & 0.83          & 0.50     \\
%     \toprule
%     \end{tabular}
%     % \end{subtable}
    
%     % \end{small}
%     \end{center}
%     \caption{Sample quality comparison with state-of-the-art generative models for each task.}
    
%     \label{tab:sota}
% \end{table*}

==> Entropy-driven Sampling and Training Scheme for Conditional Diffusion Generation(ECCV2022)/table/unconditional-ADM.tex <==
% \setlength{\tabcolsep}{4pt}
\begin{table}[!t]
% \begin{center}
    % \setlength{\tabcolsep}{6pt}
    % \vskip -0.3in
    \caption{Effect of our proposed methods based on UADM-G under DDIM 25 steps and DDPM 250 steps on ImageNet1000 256$\times$256.}
    \label{tab:unconditional}
    \begin{center}
    % \begin{small}
    \setlength{\tabcolsep}{1.8mm}{
    \begin{tabular}{cccccccc}
    \toprule
    DDIM & ECT & EDS & FID $\downarrow$   & sFID $\downarrow$ & IS $\uparrow$  & Precision $\uparrow$ & Recall $\uparrow$  \\
    \midrule
         &  &      & 12.0 & 10.4  & 95.41  & 0.76      & 0.44 \\
         & \cmark &   & 10.79 & 10.49 & 117.56  & 0.79      & 0.41 \\
         &   & \cmark  & 7.98 & 10.61 & \bf 178.73  & \bf 0.82      & 0.40 \\
         &  \cmark & \cmark & \bf 6.78 & \bf 6.56 & 168.78  & 0.81      & \bf 0.45 \\
    \hline
    \cmark     &  &      & 14.21 & 8.53  & 83  & 0.7      & \bf 0.46 \\
    \cmark     & \cmark &   & 12.21 & 8.14 & 100.95  & 0.74      & 0.44 \\
    \cmark     &  & \cmark   & 10.09 & 6.86 & 133.71  & 0.73      & 0.45 \\
    \cmark     &  \cmark & \cmark & \bf 8.28 & \bf 6.37 & \bf 163.17  & \bf 0.76      & 0.44 \\
    \bottomrule
    \end{tabular}
    }
    % \end{small}
    \end{center}
    \vspace{-2mm}
% \end{center}
\end{table}

==> algorithm/entropy-DDIM-sampling.tex <==
\algrenewcommand\algorithmicindent{0.5em}%
\begin{algorithm}[t]
    \caption{\small{Entropy-driven sampling scheme (DDIM), given a pretrained diffusion model $\epsilon_{\theta}(\bx_t)$, classifier $p_{\phi}(\tilde \by_t|\bx_t)$, and desired class condition $y$.}}
    \label{alg:entropy_driven_ddim}
    \begin{algorithmic}[1]
        \State $\bx_T \sim \mathcal{N}(\bzero, \bI)$
        \For{$t=T, \dotsc, 1$}
            % \State $\bz \sim \mathcal{N}(\bzero, \bI)$ if $t > 1$, else $\bz = \bzero$
            \State $\hbepsilon = \bepsilon_{\theta}(\bx_t) - \gamma * \frac{\mathcal{H}(\mathcal{U}(\tilde \by))}{\mathcal{H}(p_{\phi}(\tilde \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t),$
            \State $\bx_{t-1} = \sqrt{\bar \alpha_{t-1}}(\frac{\bx_t - \sqrt{1- \bar \alpha_t}\hbepsilon}{\sqrt{\bar \alpha_t}}) 
            + \sqrt{1-\bar \alpha_{t-1}}\hbepsilon$
            % \State $\bx_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left( \bx_t - \frac{1-\alpha_t}{\sqrt{1-\bar\alpha_t}} \hbepsilon_\theta(\bx_t) \right) + \sigma^2_t \bg + \sigma_t \bz$
        \EndFor
        \State \textbf{return} $\bx_0$
    \end{algorithmic}
\end{algorithm}


==> algorithm/entropy-DDPM-sampling.tex <==
\algrenewcommand\algorithmicindent{0.5em}%
\begin{algorithm}[t]
    \caption{ \small{Entropy-driven sampling scheme (DDPM), given a pretrained diffusion model $\epsilon_{\theta}(\bx_t)$, classifier $p_{\phi}(\hat \by_t|\bx_t)$, and desired class condition $\by$.}}
    \label{alg:entropy_driven_ddpm}
    \begin{algorithmic}[1]
        \State $\bx_T \sim \mathcal{N}(\bzero, \bI)$
        \For{$t=T, \dotsc, 1$}
            \State $\bz \sim \mathcal{N}(\bzero, \bI)$ if $t > 1$, else $\bz = \bzero$
            \State $\bg = \gamma * \frac{\mathcal{H}(\mathcal{U}(\hat \by))}{\mathcal{H}(p_{\phi}(\hat \by|\bx_t))} \nabla_{\bx_t} \log p_{\phi}(\by|\bx_t),$
            \State $\bx_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left( \bx_t - \frac{1-\alpha_t}{\sqrt{1-\bar\alpha_t}} \bepsilon_\theta(\bx_t) \right) + \sigma^2_t \bg + \sigma_t \bz$
        \EndFor
        \State \textbf{return} $\bx_0$
        % \RETURN $\phi$
    \end{algorithmic}
\end{algorithm}


==> algorithm/test.tex <==
\begin{algorithm}[t]
 \caption{\textbf{\label{alg:GraphBuild}}Inference graph building}
 {

 \textbf{\small{{Input:}}}{\small{
 CNN $CN$, a set $\Omega$ of images predicted by $CN$ to class $m$, network model ${\{ \Theta^l, \hat{P}(h^l=k), \hat{P}(h^l=k|h^{l'}=k')  \}}_{l=1, k=1,k'=1}^{L,K^l,K^{l'}}$,
$Z$ - number of allowed nodes per layer.
 \textbf{\small{Output:}}{
 \small{An inference graph $G=(N,E)$, where $N$ and $E$ hold clusters (nodes) and their weighted connections (edges) in the graph, respectively
 %with 

 %$N=C^L_m \cup  {\{ C^l_{z^l_i}  \}}_{l=1, i=1}^{L-1,Z}$ and 
 %$E={\{e^l_{i,j}\}}_{l=1,i=1,j=1}^{L-1,Z,Z}$ 
  }} 

 \textbf{\small{Initialization:}} 
 Push $\Omega$ through the network model to get ${\{ Q^l_{t,s}(\Omega)\}}_{l=1}^{L-1}$ (Eq.~\ref{eq:Q_t,s(omega)}) and clusters ${\{C^l_i\}}_{l=1,i=1}^{L,K^l}$.
~{\small
Set $S=m$, $N=C^L_m$, and $E=\emptyset$ %//m is the index of the output cluster to explain }
%\quad $N=S$ } 
 
 {\small For $l=L-1,\dots, 1$ }
 
% {\small{{$~~~$ Set $l= l'+1$  }}}

 {\small{{$~~~$ For $t=1,\dots,K^{l}$}}}, {\small{compute $S^{l}(\Omega,S,t)$ (Eq.~\ref{eq:OmageScore})}}

 {\small{{$~~~$ Choose $(z^{l}_1,\dots,z^{l}_Z)$ to be the $Z$ clusters indices with the largest scores $S^{l}(\Omega,S,t)$  }}}

 {\small{$~~~$ Set $S= (z^{l}_1,\dots,z^{l}_Z)$ and  $e^{l}_{i,j} = S^{l}(\Omega,z^{l+1}_i,z^{l}_j)$, $\forall i,j=1,\dots Z$ } }
 
 {\small{$~~~$ Set $N=N\cup{\{C^l_{z^l_i}\}}_{i=1}^Z$ and $E=E\cup{\{e^l_{i,j}\}}_{i=1,j=1}^{Z,Z}$ }}// nodes and edges update
%\quad $N= N \cup S$}}

% {\small{{$~~~$ Set $N= N \cup S$  }}}
  }}} }
 \end{algorithm}

==> figure/compared_ddpm250.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/compared_baseline.pdf}
         \caption{$y=x$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/compared_ECT+EDS.pdf}
         \caption{$y=3sinx$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{0.3\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{graph3}
    %      \caption{$y=5/x$}
    %      \label{fig:five over x}
    %  \end{subfigure}
        \caption{Three simple graphs}
        \label{fig:three graphs}
\end{figure}

==> figure/finegrained_feature.tex <==
\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=1.0\textwidth]{figure/finegrained_feature.jpg}
    \caption{vanishing fine-grained feature in normal inference}\label{fig:finegrained_feature}
    \end{center}
    \vskip -0.2in
\end{figure}

==> table/sota128-64.tex <==
\begin{table}[t]
    \setlength\tabcolsep{2.5mm}
    \caption{\textbf{Comparison results with state-of-the-art generative models based on ImageNet 128$\times$128, 64$\times$64.} Annotation '(25 )' after the method means its sampling process is based on DDIM with 25 steps. Otherwise, it means the normal sampling method in DDPM, with 250 steps.}
    \label{tab:sota_lowr}
    \begin{center}
    % \small
    % \begin{small}
    
    % \begin{subtable}[t]
    \begin{tabular}[t]{lcccc}
    \toprule
    Method            & FID $\downarrow$         & sFID  $\downarrow$     & Prec  $\uparrow$    & Rec $\uparrow$ \\
    \\
    \multicolumn{5}{l}{\bf{ImageNet} 64$\times$64} \\
    \toprule
    BigGAN-deep \cite{bigbigan}    & 4.06         & 3.96      & \bf{0.79} & 0.48  \\
    IDDPM    \cite{improved} & 2.92         & \bf{3.79} & 0.74      & 0.62 \\
    % CADM-G             & 2.61         & \bf{3.77} & 0.73      & 0.63  \\
    \toprule
    CADM-G  \cite{dhariwal2021diffusion} & 2.07   & 4.29      & 0.74      & \bf{0.63}  \\
    \bf{CADM-G+EDS+ECT}                & \bf{1.88}	 & 4.51     & 0.76          & 0.61          \\
    % \toprule
    % \begin{subtable}[t]{.5\linewidth}
    % \begin{tabular}[t]{lcccc}
    % \toprule
    % Model            & FID          & sFID       & Prec & Rec \\
    \\
    \multicolumn{5}{l}{\bf{ImageNet} 128$\times$128} \\
    
    \toprule
    BigGAN-deep  \cite{bigbigan}           & 6.02          & 7.18          & \bf{0.86}     & 0.35          \\
    LOGAN   \cite{logan} & 3.36          &               &               &               \\
    CADM    \cite{dhariwal2021diffusion}                     & 5.91          & 5.09     & 0.70          & \bf{0.65}     \\
    \toprule
    CADM-G (25)   \cite{dhariwal2021diffusion}   & 6.58          & 7.52          & 0.77          & 0.50          \\
    \bf{CADM-G+EDS+ECT (25)}                & 6.22	 & 7.10     & 0.78          & 0.49          \\
    % \toprule
    CADM-G    \cite{dhariwal2021diffusion}            & 2.97	 & \bf{5.09}     & 0.78          & 0.59          \\
    \bf{CADM-G+EDS+ECT}                & \bf{2.68}	 & 5.10     & 0.80          & 0.56        \\
    \toprule
    
    \end{tabular}
    % \end{subtable}
    % \begin{subtable}[t]{.5\linewidth}
    % \begin{tabular}[t]{lcccc}
    
    % \toprule
    % Method            & FID $\downarrow$         & sFID  $\downarrow$     & Prec  $\uparrow$    & Rec $\uparrow$ \\
    % \\
    
    % \multicolumn{5}{l}{\bf{ImageNet} 256$\times$256} \\
    % \toprule
    % DCTransformer            & 36.51         & 8.24          & 0.36          & \bf{0.67}  \\

    % VQ-VAE-2 & 31.11 & 17.38 & 0.36 & 0.57 \\
    % IDDPM & 12.26 & 5.42 & 0.70 & 0.62 \\
    % SR3 & 11.30 & & & \\
    % BigGAN-deep             & 6.95          & 7.36          & \bf{0.87}     & 0.28       \\
    % UADM-G  (25)                & 14.21         & 8.53          & 0.7          & 0.46       \\
    % UADM-G                & 12         & 10.4          & 0.76          & 0.44       \\
    % CADM                  & 10.94         & 6.02          & 0.69          & 0.63       \\
    % CADM-G (25)    & 5.44	         & 5.32          & 0.81	         & 0.49       \\
    % CADM-G              & 4.59     & 5.25     & 0.82          & 0.52       \\
    % \toprule
    % \bf{UADM-G + ECT + EDS} (25)                & 8.28      & 6.37     & 0.76          & 0.44     \\
    % \bf{UADM-G + ECT + EDS}            & 6.78     & 6.56     & 0.81          & 0.45     \\
    % \bf{CADM-G + ECT + EDS} (25)                & 4.67      & 5.12     & 0.82          & 0.47     \\
    % \bf{CADM-G + ECT + EDS}            & \bf{4.09}     & \bf{5.07}     & 0.83          & 0.50     \\
    % \toprule
    % \end{tabular}
    % \end{subtable}
    
    % \end{small}
    \end{center}
    
    
    
    \vskip -0.2in
\end{table}



% \begin{table*}[th]
%     \setlength\tabcolsep{6pt}
%     \begin{center}
%     % \begin{small}
    
%     % \begin{subtable}[t]{.5\linewidth}
%     % \setlength{\tabcolsep}{5mm}{
%     \begin{tabular}[t]{lcccc}
%     \toprule
%     Method            & FID $\downarrow$         & sFID  $\downarrow$     & Precision  $\uparrow$    & Recall $\uparrow$ \\
    
%     % \multicolumn{5}{l}{\bf{ImageNet} 256$\times$256} \\
%     \toprule
%     DCTransformer${}^\dagger$ \cite{dctransformer}            & 36.51         & 8.24          & 0.36          & \bf{0.67}  \\
%     % IDDPM \shortcite{improved} & 31.50 & 20.27 & 0.65 & 0.60 \\
    
%     % VQ-VAE-2 vqvae2
%     % IDD improved
%     % sr3 sr3
%     % Biggan biggan
%     % ADM dhariwal
%     VQ-VAE-2${}^\dagger{}^\ddag$ \cite{vqvae2} & 31.11 & 17.38 & 0.36 & 0.57 \\
%     IDDPM${}^\ddag$ \cite{improved} & 12.26 & 5.42 & 0.70 & 0.62 \\
%     SR3${}^\dagger{}^\ddag$ \cite{sr3} & 11.30 & & & \\
%     BigGAN-deep \cite{biggan}             & 6.95          & 7.36          & \bf{0.87}     & 0.28       \\
%     ADM      \cite{dhariwal2021diffusion}            & 10.94         & 6.02          & 0.69          & 0.63       \\
%     ADM-G (25 steps)  \cite{dhariwal2021diffusion}  & 5.44	         & 5.32          & 0.81	         & 0.49       \\
%     ADM-G    \cite{dhariwal2021diffusion}          & 4.59     & 5.25     & 0.82          & 0.52       \\
%     \toprule
%     \bf{ADM-EDT} (25 steps)                     & 5.34         & 5.3         & 0.81          & 0.49      \\
%     \bf{ADM-EDT}      & 4.62	         & 5.16         & 0.81	         & 0.53       \\
%     \bf{ADM-EDT + EDS} (25 steps)                & 4.81      & 5.22     & 0.83          & 0.45     \\
%     \bf{ADM-EDT + EDS}             & \bf{4.09}     & \bf{5.07}     & 0.83          & 0.50     \\
%     \toprule
%     \end{tabular}
%     % \end{subtable}
    
%     % \end{small}
%     \end{center}
%     \caption{Sample quality comparison with state-of-the-art generative models for each task.}
    
%     \label{tab:sota}
% \end{table*}
